Thermodynamic Formalism for Generalized Countable Markov Shifts

Countable Markov shifts, denoted by $\Sigma_A$ for a 0-1 infinite matrix $A$, are central objects in symbolic dynamics and ergodic theory. R. Exel and M. Laca introduced the corresponding operator algebras, a generalization of the Cuntz-Krieger algebras for infinite countable alphabet, and the set $X_A$, a kind of Generalized Markov Shift (GMS) that coincides with $\Sigma_A$ in the locally compact case. The set $\Sigma_A$ is dense in $X_A$, and its complement, a set of finite allowed words, is dense in $X_A$ when non-empty. We develop the thermodynamic formalism for $X_A$, introducing the notion of conformal measure in it, and exploring its connections with the usual formalism for $\Sigma_A$. New phenomena appear, as different types of phase transitions and new conformal measures undetected by the classical thermodynamic formalism for $A$ not row-finite. Given a potential $F$ and inverse of temperature $\beta$, we study the existence of conformal measures $\mu_{\beta}$ associated to $\beta F$. We present examples where there exists a critical $\beta_c$ s. t. we have existence of conformal probabilities satisfying $\mu_{\beta}(\Sigma_A)=0$ for every $\beta > \beta_c$ and, on the weak$^*$ topology, the set of conformal probabilities for $\beta >\beta_c$ collapses to the standard conformal probability $\mu_{\beta_c}$, $\mu_{\beta_c}(\Sigma_A)=1$, for the limit $\beta\to\beta_c$. We study in detail the generalized renewal shift and modifications of it. We highlight the bijection between infinite emitters of the alphabet and extremal conformal probabilities for this class of renewal type shifts. We prove the existence and uniqueness of the eigenmeasure probability of the Ruelle's transformation at low enough temperature for a particular potential on the generalized renewal shift; such measures are not detected on the standard renewal shift since for low temperatures, $\beta F$ is transient.

==> KMS.tex <==

\section{KMS states}

\label{section:kms}
%Before we state the second Neshveyev's theorem, we define KMS states. The results in this section can be found in \cite{frausino2018}.
In this section we define the notion of KMS states and prove some of their main properties. The results in this section can be found in \cite{bratteli2012operator}, \cite{bratteli1996operator} and \cite{Frausino2018}. KMS states characterizes the equilibrium states in quantum statistical mechanics.

Before we define KMS states, let us recall the definition of approximate unit and prove some properties of states on a C$^*$-algebra.


Recall the following theorems on positive linear functionals from \cite{murphy2014c}:
\begin{theorem} %Murphy T 3.3.1 pg 88
\label{thm:positivefunctionalbounded}
If $\varphi$ is a positive linear functional on a C$^*$-algebra $A$, then it is bounded.
\end{theorem}

\begin{theorem} %Murphy T 3.3.3 pg 88
\label{thm:stateapproximateunit}
Let $\varphi$ be a bounded linear functional on a C$^*$-algebra $A$. The following conditions are equivalent:
\begin{itemize}
\item $\varphi$ is positive.
\item For each approximate unit $\{ u_\lambda \}_{\lambda \in \Lambda}$, $\Vert \varphi \Vert = \lim_{\lambda} \varphi(u_\lambda)$.
\item For some approximate unit $\{ u_\lambda \}_{\lambda \in \Lambda}$, $\Vert \varphi \Vert = \lim_{\lambda} \varphi(u_\lambda)$.
\end{itemize}
\end{theorem}
\begin{proof}
Assume $\varphi \neq 0$. First we show the implication $(i) \Rightarrow (ii)$ holds.

Note that the map $A^2 \rightarrow \mathbb{C}$ defined by $(a,b) \mapsto \varphi(b*a)$ is a positive sesquilinear form on $A$. Hence $\varphi(b*a) = \overline{\varphi(a*b)}$ and the Cauchy-Schwarz inequality $\vert \varphi(b*a) \vert \leq \varphi(b*b)^{1/2} \varphi(a*a)^{1/2}$ holds.

Let $(u_\lambda)_{\lambda \in \Lambda}$ be an approximate unit of $A$ and let $a \in A$ with $a \neq 0$. Then, for every $\lambda \in \Lambda$,
\begin{align}
\label{eqn:varphiulambda}
\vert \varphi(au_\lambda) \vert^2
\leq \varphi(a*a) \varphi(u_\lambda * u_\lambda )
=    \varphi(a*a) \varphi(u_\lambda^2),
\end{align}
by the Cauchy-Schwarz inequality. Since the net $\{ u_\lambda \}_{\lambda \in \Lambda}$ is increasing and its elements are in the unit ball, then the net $\{ u_\lambda^2 \}_{\lambda \in \Lambda}$ is also increasing and included in the unit ball. Because $\varphi$ is positive and bounded, we have
$\sup_{\lambda \in \Lambda} \varphi(u_\lambda^2) = \lim_{\lambda \in \Lambda} \varphi(u_\lambda^2)$. Then, for every $i \in \Lambda$, we have by $\eqref{eqn:varphiulambda}$,
\begin{align*}
\vert \varphi(au_i) \vert^2
\leq \varphi(a*a) \lim_{\lambda \in \Lambda} \varphi(u_\lambda^2)
\leq \Vert \varphi \Vert \Vert a*a \Vert \lim_{\lambda \in \Lambda} \varphi(u_\lambda^2)
= \Vert \varphi \Vert \Vert a \Vert^2 \lim_{\lambda \in \Lambda} \varphi(u_\lambda^2).
\end{align*}
Therefore, using the continuity of $\varphi$,
\begin{align*}
\lim_{\lambda \in \Lambda} \vert \varphi(au_i) \vert^2 \leq \Vert \varphi \Vert \Vert a \Vert^2 \lim_{\lambda \in \Lambda} \varphi(u_\lambda^2)\\
\vert \varphi(a) \vert^2 \leq \Vert \varphi \Vert \Vert a \Vert^2 \lim_{\lambda \in \Lambda} \varphi(u_\lambda^2)\\
\frac{\vert \varphi(a) \vert^2}{\Vert a \Vert^2 } \leq \Vert \varphi \Vert \lim_{\lambda \in \Lambda} \varphi(u_\lambda^2).
\end{align*}
Since $a$ is arbitrary, $\Vert \varphi \Vert \leq \lim_{\lambda \in \Lambda} \varphi(u_\lambda^2)$. On the other hand, for each $\lambda \in \Lambda$,
\begin{align*}
\varphi(u_\lambda^2)
\leq \Vert \varphi \Vert \Vert u_\lambda^2 \Vert
\leq \Vert \varphi \Vert.
\end{align*}
Then $\Vert \varphi \Vert = \lim_{\lambda \in \Lambda} \varphi(u_\lambda^2)$. Note that $u_\lambda^2 - u_\lambda \leq 0$ for every $\lambda$, thus $\varphi(u_\lambda^2) \leq \varphi(u_\lambda)$. Therefore,
\begin{align*}
\Vert \varphi \Vert
= \lim_{\lambda \in \Lambda} \varphi(u_\lambda^2)
\leq \lim_{\lambda \in \Lambda} \varphi(u_\lambda)
\leq \Vert \varphi \Vert.
\end{align*}

It is obvious that $(ii) \Rightarrow (iii)$.

Now we show that $(iii) \Rightarrow (i)$. Suppose that $\{ u_n \}_{n \in \mathbb{N}}$ is an approximate unit such that $1 = \lim_{n \rightarrow \infty} \tau(u_n)$. Let $a$ be a selft-adjoint element of $A$ such that $\Vert a \Vert \leq 1$ and write $\tau(a) = \alpha + i\beta$ where $\alpha$, $\beta$ are real numbers. To show that $\tau(a) \in \mathbb{R}$, we may suppose that $\beta \leq 0$. If $k$ is a positive integer, then
\begin{align*}
\Vert a - iu_\lambda \Vert^2
&= \Vert (a + iku_n)(a - iku_n)\Vert\\
&= \Vert a^2 +k^2 u_n^2 - ik(au_n - u_na) \Vert\\
&\leq 1 + k^2 + k \Vert au_n - u_n a \Vert
,
\end{align*} so $\vert \tau(a - iku_n) \vert^2 \leq 1 + k^2 + k \Vert au_n - u_na \Vert$ because $\Vert \tau \Vert = 1$.

However, $\lim_{k \rightarrow \infty} \tau(a - iku_n) = \tau(a) - ik$ by hypothesis, and $\lim_{k \rightarrow \infty} (a u_n - u_n a) = 0$, so in the limit as $n \rightarrow \infty$, we get
\begin{align*}
\vert \alpha + i\beta - ik \vert^2
= \vert \tau(a) - ik\vert^2
= \vert \alpha + i\beta -ik \vert^2
\leq 1 + k^2,
\end{align*}
then
\begin{align*}
&\alpha^2 + \beta^2 -2k\beta + k^2 \leq 1 + n^2\\
\Rightarrow & -2k\beta \leq 1 - \beta^2 - \alpha^2.
\end{align*}
Since $\beta$ is not positive and this inequality holds for all positive integers $n$, $\beta$ must be zero. Therefore, $\tau(a)$ is real if $a$ is hermitian.

Now suppose that $a$ is positive and $\Vert a \Vert \leq 1$. Then $u_n - a$ is hermitian and $\Vert u_n - a \Vert \leq 1$, so $\tau(u_n - a) \leq 1$. But then $1 - \tau(a) = \lim_{n \rightarrow \infty} \tau(u_n - a) \leq 1$, and therefore $\tau(a) \geq 0$. Thus, $\tau$ is positive and we have shown $(iii) \Rightarrow (i)$.
\end{proof}

%%%\begin{remark}
%%%\label{remark:stateconvex}
%%%Note that the set of states is convex. In fact, given $\varphi_1, \varphi_2$ states on a C$^*$-algebra, $0 < t < 1$, let $\varphi = t \varphi_1 + (1-t)\varphi_2$. It follows that $\varphi$ is positive. Let $\{ u_\lambda \}_{\lambda \in \Lambda}$ be an approximate unit of $A$. It follows from Theorem \ref{thm:stateapproximateunit} that
%%%\begin{align*}
%%%\Vert \varphi \Vert
%%%&= \lim_\lambda \varphi(u_\lambda)\\
%%%&= \lim_\lambda [t\varphi_1(u_\lambda) + (1-t)\varphi_2(u_\lambda)]\\
%%%&= [t\Vert \varphi_1 \Vert + (1-t)\Vert \varphi_2 \Vert]\\
%%%&= t + (1-t)\\
%%%&= 1.
%%%\end{align*}
%%%Then $\varphi$ is a state.
%%%\end{remark}

We want to show that, if the C$^*$-algebra $A$ is commutative and unital, then the extremal states are precisely the characters on $A$. We need some results on convex spaces before studying this. 

\begin{definition} %Murphy pg 14
Given a commutative C$^*$-algebra $A$, a {character} is a non-zero homomorphism $\varphi: A \rightarrow \mathbb{C}$.
\end{definition}

\begin{definition}
Let $X$ be a normed vector space. A functional $\eta$ in a convex subset $C \subset X*$ is an {extreme point} in $C$ (or {extremal}) if the condition $\eta = t\eta_1 + (1-t)\eta_2$, where $\eta_1, \eta_2 \in C$, $0 < t < 1$, implies that $\eta = \eta_1 = \eta_2$.
\end{definition}

\begin{definition} %\Murphy pg 144
We say that a state $\varphi$ on $A$ is {pure} if it has the property that whenever $\rho$ is a positive linear functional on $A$ such that $\rho \leq \varphi$, necessarily there is a number $t \in [0,1]$ such that $\rho = t\varphi$.
\end{definition}

\begin{theorem}\cite[Theorem 2.3.15]{bratteli1996operator} %Ver rascunho no caderno
Let $A$ be a unital C$^*$-algebra. The set of states on $A$ is convex and its extremal points are the pure states.
\end{theorem}

\begin{theorem}\cite[Theorem 5.1.6]{murphy2014c} %pg 144
Let $\varphi$ be a state on a commutative C$^*$-algebra $A$. Then $\varphi$ is pure if, and only if, it is a character on $A$.
\end{theorem}

\begin{lemma}
\label{lemma:integralofstates}
Let $X$ be a Borel space endowed with a probability measure $\mu$. Let $A$ be a separable C$^*$-algebra and $A_0$ a dense subset of $A$. Let $\psi_x$ be a family of states on $A$ defined for $\mu$-a.e. $x \in X$ such that for every $a \in A_0$ the map $x \mapsto \psi_x(a)$ is $\mu$-measurable. Define $\varphi$ by
\begin{align*}
\varphi(a) = \int_X \psi_x(a) d\mu(x)
.
\end{align*}
Then $\varphi$ is a state on $A$.
\end{lemma}
\begin{proof}
Let $V \subset X$ be a conull set such that $\psi_x$ is defined for every $x \in V$. Define for every $a \in A$ the function $F_a: X \rightarrow \mathbb{C}$ by
\begin{align*}
F_a(x) =
\begin{cases}
\psi_x(a) & \text{if $x \in V$}\\
0 & \text{otherwise.}
\end{cases}
\end{align*}
By assumption, $F_a$ is $\mu$-measurable for every $a \in A_0$.

Let $a \in A$. Since $A_0$ is dense in $A$, there exists a sequence $\{ a_n \}_{n \in \mathbb{N}}$ in $A_0$ converging to $a$. Then, using the continuity of $\psi_x$, we have for $\mu$-a.e. $x$,
\begin{align*}
F_a(x) = \psi_x(a) = \lim_{n \rightarrow \infty} \psi_x(a_n) = \lim_{n \rightarrow \infty} F_{a_n}(x).
\end{align*}
Therefore $F_a$ is measurable. In other words, the function $x \mapsto \psi_x(a)$ is $\mu$-measurable for every $a \in A$.

In order to show that $\varphi$ is a state, we begin by proving that $\varphi$ is a positive linear functional. Since each $\psi_x$ linear, it follows from the definition of $\varphi$ that $\varphi$ is also linear. Let $a$ be a positive element in $A$. Then $\psi_x(a) \geq 0$ for $\mu$-a.e. $x$. Thus,
\begin{align*}
\varphi(a) = \int_X \psi_x(a) d\mu(x) \geq 0.
\end{align*}
By Theorem \ref{thm:positivefunctionalbounded}, $\varphi$ is bounded. It follows from Theorem \ref{thm:stateapproximateunit} that, for some approximate unit $\{ u_n \}_{n \in \mathbb{N}}$ of $A$,
\begin{align*}
\Vert \varphi \Vert
= \lim_{n \rightarrow \infty} \varphi(u_n)
= \lim_{n \rightarrow \infty} \int_X \psi_x(u_n)d\mu(x).
\end{align*}
However,
\begin{align*}
\vert \psi_x(u_n) \vert \leq \Vert \psi_x \Vert \Vert u_n \Vert = \Vert u_n \Vert \leq 1,
\end{align*}
for every $n$ and for $\mu$-a.e. $x \in X$ because each $\psi_x$ is a state and every $u_n$ satisfies $\Vert u_n \Vert \leq 1$. Therefore we can apply the dominated convergence theorem, then
\begin{align*}
\Vert \varphi \Vert
&= \lim_{n \rightarrow \infty} \int_X \psi_x(u_n) d\mu(x)\\
&= \int_X \left( \lim_{n \rightarrow \infty} \psi_x(u_n) \right) d\mu(x)\\
&= \int_X 1 d\mu(x), \text{\hspace{10pt} since each $\psi_x$ is a state,}\\
&= 1.
\end{align*}
\end{proof}

Now we define the notion of dynamical system on a C$^*$-algebra and prove some of its properties.

\begin{definition} %pg 11 frausino
\label{def:groupofautomorphisms}
We say that $\tau = \{ \tau_t \}_{t \in \mathbb{R}}$ is a {one-parameter group of $\ast$-automorphisms} of a C$^*$-algebra $A$ if $\tau_t: A \rightarrow A$ is an $\ast$-automorphism and
\begin{itemize}
\item $\tau_{t+s} = \tau_t \circ \tau_s$ for all $t, s \in \mathbb{R}$;
\item $\tau_0 = id$.
\end{itemize}
\end{definition}

\begin{example}
Consider the algebra of square matrices $M_n(\mathbb{C})$ for some $n$. Let $H \in M_n(\mathbb{C})$, and define each $\tau_t: M_n(\mathbb{C}) \rightarrow M_n(\mathbb{C})$ by $\tau_t(A) = e^{itH}Ae^{-itH}$. Note that $\tau_t$ is linear and $\tau_0$ is the identity. Each $\tau_t$ is a homomorphism because
\begin{align*}
\tau_t(AB)
= e^{itH}ABe^{-itH}
= e^{itH}Ae^{-itH}e^{itH}Be^{-itH}
= \tau_t(A)\tau_t(B).
\end{align*}
Also, the equality $\tau_{t+s} = \tau_t \circ \tau_s$ holds, since
\begin{align*}
\tau_{t+s}(A)
= e^{i(t+s)H}Ae^{-i(t+s)H}
= e^{itH}e^{isH}Ae^{-isH}e^{-itH}
= e^{itH}\tau_s(A)e^{-itH}
= \tau_t(\tau_s(A)).
\end{align*}
\end{example}

\begin{definition} %D 12 pg 11 frausino
A {C$^*$-dynamical system} is a pair $(A, \tau)$ where $A$ is a C$^*$-algebra and $\tau = \{ \tau_t \}_{t \in \mathbb{R}}$ is a one-parameter group of $\ast$-automorphisms {strongly continuous}, i.e., $t \mapsto \tau_t(a)$ is continuous in the norm for all $a \in A$. If we fix $\tau$, we say that $\tau$ is the {dynamics} on $A$.
\end{definition}

%Now we prove that, in order to show that one-parameter group of $\ast$-automorphisms is a dynamics, it is sufficient to prove the continuity of $t \mapsto \tau_t(a)$ for a dense $\ast$-subalgebra of $A$ if $\Vert \tau_t(a) \Vert \leq \Vert a \Vert$.

Now we prove that, under certain conditions, if we define a one-parameter group of $\ast$-automorphisms $\tau$ on a dense $\ast$-algebra of a C$^*$-algebra $A$, then we can extend the operators uniquely on $A$. Moreover, $\tau$ defines a dynamics on $A$.

\begin{lemma} %eu com ajuda do frausino
\label{lemma:dynamicsextension}
%Let $\tau = \{ \tau_t \}_{t \in \mathbb{R}}$ be a one-parameter group of $\ast$-automorphisms of a
Let $A_0$ be a dense $\ast$-subalgebra of a C$^*$-algebra $A$. Let $\tau = \{ \tau_t \}_{t \in \mathbb{R}}$ be a family of $\ast$-automorphisms $\tau_t : A_0 \rightarrow A_0$ such that
\begin{itemize}
\item $\tau_{t+s} = \tau_t \circ \tau_s$ for $t,s \in \mathbb{R}$,
\item $\tau_0 = id$,
\item $t \mapsto \tau_t(a)$ is continuous in the norm for each $a \in A_0$.
\end{itemize}
Moreover, assume
\begin{align}
\label{eqn:tauboundedonA0}
\Vert \tau_t(a) \Vert \leq \Vert a \Vert,
\text{\hspace{10pt} for every $t \in \mathbb{R}, a \in A_0$.}
\end{align}
Then $\tau$ can be extended uniquely to a dynamics on $A$, which we also denote by $\tau = \{ \tau_t \}_{t \in \mathbb{R}}$ without loss of generality.
\end{lemma}
\begin{proof}
First we show that each $\tau_t$ can be extended uniquely to $A$. Let $a \in A$. Since $A_0$ is dense in $A$, there exists a sequence $\{ a_n \}_{n \in \mathbb{N}}$ converging to $a$.

Using the fact that $A_0$ is a vector space and the equation $\eqref{eqn:tauboundedonA0}$, we have that $\{ \tau_t(a_n)\}_{n \in \mathbb{N}}$ is a Cauchy sequence, then we can define $\tau_t(a) = \lim_{n \rightarrow \infty} \tau_t(a_n)$.

Note that $\tau_t(a)$ is well-defined. In fact, let $\{ b_n \}_{n \in \mathbb{N}}$ be an arbitrary sequence converging to $a$, and let $x = \lim_{n \rightarrow \infty} \tau_t(b_n)$. Then
\begin{align*}
\Vert \tau_t(a) - x \Vert
= \lim_{n \rightarrow \infty} \Vert \tau_t(a_n) - \tau_t(b_n) \Vert
\leq \lim_{n \rightarrow \infty} \Vert a_n - b_n \Vert
= 0.
\end{align*}

It follows from the defintion of $\tau_t$ on $A$ that $\Vert \tau_t(a) \Vert \leq \Vert a \Vert$ for every $a \in A$.

Note that the extension $\tau$ also satisfies $\tau_0 = id$ and $\tau_{t+s} = \tau_t \circ \tau_s$. In fact, given $a \in A$, let $\{ a_n \}_{n \in \mathbb{N}}$ be a sequence in $A_0$ converging to $a$. Then
\begin{align*}
\tau_0(a)
&= \lim_{n \rightarrow \infty} \tau_0(a_n)
= \lim_{n \rightarrow \infty} a_n
= a\\
\tau_{t+s}(a)
&= \lim_{n \rightarrow \infty} \tau_{t+s}(a_n)
= \lim_{n \rightarrow \infty} \tau_t \circ \tau_s(a_n)
= \tau_t \circ \tau_s(a).
\end{align*}
Then $\tau_t$ is invertible with inverse $\tau_{-t}$.

Now we show that $\tau_t: A \rightarrow A$ is an automorphism. Let $a,b \in A$ and $\{ a_n \}_{n \in \mathbb{N}},\{ b_n \}_{n \in \mathbb{N}}$ sequences in $A_0$ converging to $a, b$ respectively. Then
 \begin{align*}
 \tau_t(ab)
 &= \lim_{n \rightarrow \infty} \tau_t(a_nb_n)
 = \lim_{n \rightarrow \infty} \tau_t(a_n)\tau_t(b_n)
 =\tau_t(a)\tau_t(b),\\
 \tau_t(a*)
 &= \lim_{n \rightarrow \infty} \tau_t(a_n*)
 = \lim_{n \rightarrow \infty} \tau_t(a_n)*
 = \tau_t(a)*.
 \end{align*}
Finally, we show that $\tau$ is strongly continuous. Let $a \in A$ and fix $t_0$. Given $\varepsilon$, there exists $a_0 \in A_0$ such that $\Vert a - a_0 \Vert < \varepsilon/3$. Let $\delta > 0$ such that $\Vert \tau_t(a_0) - \tau_s(a_0) \Vert < \varepsilon/3$ for every $t \in \mathbb{R}$ such that $\vert t - t_0 \vert < \delta$.

Given $t$ with $\vert t - t_0 \vert < \delta$, we have
\begin{align*}
\Vert \tau_t(a) - \tau_{t_0}(a) \Vert
&\leq \Vert \tau_t(a) - \tau_t(a_0) \Vert
+ \Vert \tau_t(a_0) - \tau_{t_0}(a_0) \Vert + \Vert \tau_{t_0}(a_0) - \tau_{t_0}(a) \Vert\\
&\leq 2 \Vert a - a_0 \Vert + \Vert \tau_t(a_0) - \tau_{t_0}(a_0) \Vert\\
&\leq 2 \frac{\varepsilon}{3} + \frac{\varepsilon}{3}\\
&= \varepsilon.
\end{align*}
\end{proof}


Let $X$ be a complex Banach space and $X*$ its dual. Let $\sigma(X, X*)$ denote the topology on $X$ induced by the functionals on $X$. This topology is denoted the {weak topology} on $X$.

\begin{remark}
We say that a function $f: \mathbb{R} \rightarrow X$ is $\sigma(X,X*)$-continuous if $\eta \circ f: \mathbb{R} \rightarrow \mathbb{C}$ is continuous for every $\eta \in X*$.
\end{remark}

\begin{definition} %D 12 pg 11 frausino
\label{def:groupofisometries}
Given a Banach space $X$, let $\{ \tau_t \}_{t \in \mathbb{R}}$ be a family of linear and bounded operators $\tau_t: X \rightarrow X$. This family is called a {one-parameter $\sigma(X,X*)$-continuous group of isometries} if
\begin{itemize}
\item $\tau_{t+s} = \tau_t \circ \tau_s$ for all $t, s \in \mathbb{R}$;
\item $\tau_0 = id$;
\item $\Vert \tau_t \Vert = 1$ for all $t \in \mathbb{R}$;
\item $t \mapsto \tau_t(a)$ is $\sigma(X,X*)$-continuous for all $a \in X$.
\end{itemize}
\end{definition}

\begin{lemma} %eu estou provando, conferir
Let $A$ be a C$^*$-algebra and $\tau$ its dynamics. Then $\tau$ is a one-parameter $\sigma(A,A*)$-continuous group of isometries.
\end{lemma}
\begin{proof}
%\label{def:groupofisometries}\label{def:groupofautomorphisms}
Note that properties (i) and (ii) in Definitions \ref{def:groupofautomorphisms} and \ref{def:groupofisometries} are equal. In both, every $\tau$ is a linear operator on $A$. So we need to show properties (iii) and (iv) of Definition \ref{def:groupofisometries}.

\begin{itemize}
\setcounter{enumi}{2}
\item $\Vert \tau_t \Vert = 1$

This follows from the fact that every $\ast$-automorphism on a C$^*$-algebra is an isometry.

%%%%%%%%%Consider $\widetilde{A}$ the unitization of $A$. If $A$ is unital, we assume $\widetilde{A} = A$. Otherwise, we write $\widetilde{A} = A \oplus \mathbb{C}$. More details on unitization of C$^*$-algebras can be found in \cite{murphy2014c}.
%%%%%%%%%
%%%%%%%%%Define, for every $t$, the linear operator $\widetilde{\tau}_t: \widetilde{A} \rightarrow \widetilde{A}$ such that $\widetilde{\tau}_t(a) = \tau_t(a)$ if $a \in A$, and $\tau(1) = 1$. Note that $\widetilde{\tau}_t$ is well-defined even if $A$ is unital. In this case, $\widetilde{\tau}_t = \tau_t$. In fact, let $a \in A$. Since $\tau_t$ is an automorphism, there exists $a_0 \in A$ such that $a = \tau_t(a_0)$. Thus
%%%%%%%%%\begin{align*}
%%%%%%%%%\tau_t(1) a = \tau_t(1) \tau_t(a_0) = \tau_t(1a_0) = \tau_t(a_0) = a.
%%%%%%%%%\end{align*}
%%%%%%%%%Analogously, $a \tau_t(1) = a$. Since $a$ is arbitrary, we have $1 = \tau_t(1)$.
%%%%%%%%%
%%%%%%%%%Now we show that $\widetilde{\tau}_t$ is a homomorphism for any C$^*$-algebra $A$. In fact, for $a_1 + \lambda_1, a_2 + \lambda_2 \in \widetilde{A}$,
%%%%%%%%%\begin{align*}
%%%%%%%%%\widetilde{\tau}_t((a_1 + \lambda_1 1)(a_2 + \lambda_2 1))
%%%%%%%%%&= \widetilde{\tau}_t (a_1 a_2 + \lambda_2 a_1 + \lambda_1 a_2 + \lambda_1 \lambda_2 1)\\
%%%%%%%%%&= \widetilde{\tau}_t(a_1 a_2) + \lambda_2 \widetilde{\tau}_t(a_1) + \lambda_1\widetilde{\tau}_t(a_2) + \widetilde{\tau}_t(\lambda_1 \lambda_2)
%%%%%%%%%\text{,\hspace{10pt} by linearity of $\widetilde{\tau}_t$,}\\
%%%%%%%%%&= \tau_t(a_1 a_2) + \lambda_2 \tau_t(a_1) + \lambda_1\tau_t(a_2) + \lambda_1 \lambda_2
%%%%%%%%%\text{,\hspace{10pt} by definition of $\widetilde{\tau}_t$,}\\
%%%%%%%%%&= \tau_t(a_1) \tau_t (a_2) + \lambda_2 \tau_t(a_1) + \lambda_1\tau_t(a_2) + \lambda_1 \lambda_2
%%%%%%%%%.
%%%%%%%%%\end{align*}
%%%%%%%%%On the other hand,
%%%%%%%%%\begin{align*}
%%%%%%%%%\widetilde{\tau}_t(a_1+\lambda_1)\widetilde{\tau}_t(a_2 + \lambda_2)
%%%%%%%%%&= (\tau_t(a_1) + \lambda_1)(\tau_t(a_2) + \lambda_2)\\
%%%%%%%%%&= \tau_t(a_1)\tau_t(a_2) + \lambda_2\tau_t(a_1) + \lambda_1\tau_t(a_2) + \lambda_1 \lambda_2
%%%%%%%%%.
%%%%%%%%%\end{align*}
%%%%%%%%%Hence $\widetilde{\tau}_t$ is a homomorphism. In order to show that $\tau_t$ has norm one, we will prove that $\Vert \tau_t (a)\Vert = \Vert a \Vert$. Assume $a \in A$ is self-adjoint. Let $\lambda \in r(a)$. Thus $a - \lambda$ is invertible in $\widetilde{A}$, i.e., there is $\widetilde{b} \in \widetilde{A}$ satisfying
%%%%%%%%%\begin{align*}
%%%%%%%%%(a - \lambda)\widetilde{b} = \widetilde{b} (a - \lambda) = 1.
%%%%%%%%%\end{align*}
%%%%%%%%%Then
%%%%%%%%%\begin{align*}
%%%%%%%%%\widetilde{\tau}_t \left[ (a - \lambda)\widetilde{b} \right]
%%%%%%%%%&= \widetilde{\tau}_t \left[ \widetilde{b} (a - \lambda) \right]
%%%%%%%%%= \widetilde{\tau}_t(1)\\
%%%%%%%%%\widetilde{\tau}_t(a - \lambda)\widetilde{\tau}_t(\widetilde{b})
%%%%%%%%%&= \widetilde{\tau}_t (\widetilde{b}) \widetilde{\tau}_t(a - \lambda) = 1\\
%%%%%%%%%(\tau_t(a) - \lambda)\widetilde{\tau}_t(\widetilde{b})
%%%%%%%%%&= \widetilde{\tau}_t (\widetilde{b}) (\tau_t(a) - \lambda) = 1
%%%%%%%%%.
%%%%%%%%%\end{align*}
%%%%%%%%%Hence $\lambda \in r(\tau_t(a))$. Therefore $r(a) \subset r(\tau_t(a))$. Using the fact that $a = \tau_{-t}(\tau_t(a))$, then $\tau_t(a)$ is self-adjoint since $\tau_t(a)* = \tau_t(a*) = \tau_t(a)$. Then, by the same arguments,
%%%%%%%%%\begin{align*}
%%%%%%%%%r(\tau_{t}(a)) \subset r(\tau_{-t}(\tau_{t}(a))) = r(a).
%%%%%%%%%\end{align*}
%%%%%%%%%Thus $r(\tau_t(a)) = r(a)$. Then $\Vert \tau_t(a) \Vert = \Vert a \Vert$.
%%%%%%%%%
%%%%%%%%%Now let $a \in A$ be arbitrary, then $a*a$ is self-adjoint. Hence,
%%%%%%%%%\begin{align*}
%%%%%%%%%\Vert \tau_t(a) \Vert^2
%%%%%%%%%= \Vert \tau_t(a)* \tau_t(a) \Vert
%%%%%%%%%= \Vert \tau_t(a*a) \Vert
%%%%%%%%%= \Vert a*a \Vert
%%%%%%%%%= \Vert a \Vert^2.
%%%%%%%%%\end{align*}
%%%%%%%%%Therefore $\Vert \tau_t \Vert = 1$.

\item $t \mapsto \tau_t(a)$ is $\sigma(A, A*)$-continuous for all $a \in A$

Let $a \in A$ and $t_0 \in \mathbb{R}$. $\tau$ is strongly continuous by assumption. Then $\tau_t(a) \rightarrow \tau_{t_0}(a)$ in the norm as $t \rightarrow t_0$. Thus, for every $\eta \in A*$, $\eta(\tau_t(a)) \rightarrow \eta(\tau_{t_0}(a))$ as $t \rightarrow t_0$. Thus property (iv) holds.
\end{itemize}
Therefore $\tau$ is a one-parameter $\sigma(A,A*)$-continuous group of isometries.
\end{proof}

Note that, for every $a \in X$, the function $t \mapsto \eta \circ \tau_t(a)$ is continuous for all $\eta \in X*$. If we can extend this function to an analytic function on a strip in $\mathbb{C}$ which we will define later, we say that $a$ is analytic. We will prove that the set of analytic elements is dense in $X$.

\begin{definition} %D 13 pg 11 frausino
\label{def:analytic}
Let $\tau$ be a one-parameter $\sigma(X, X*)$-continuous group of isometries. An element $a \in X$ is {analytic} for $\tau$ if there exists $\lambda > 0$ and a function $f: I_\lambda \rightarrow X$, where $I_\lambda = \{ z \in \mathbb{C} : \vert Im(z) \vert < \lambda \}$, such that
\begin{itemize}
\item $f(t) = \tau_t(a)$ for all $t \in \mathbb{R}$;
\item The function $z \mapsto \eta(f(z))$ is analytic in $I_\lambda$ for all $\eta \in X*$.
\end{itemize}

Under these conditions we write $$\tau_z(a) = f(z), \text{ for $z \in I_\lambda$}.$$

If $\lambda = \infty$, we say that $a$ is {entire analytic} for $\tau$.
\end{definition}

\begin{remark}
\label{remark:analyticvectorspace}
Suppose $a_1, a_2 \in X$ are entire analytic, and $\alpha \in \mathbb{C}$. Let $f_1, f_2$ be the corresponding functions as in Definition \ref{def:analytic}. Then, for every $t \in \mathbb{R}$,
\begin{align}
\label{eqn:entirevectorspace}
f_1(t) + \alpha f_2(t) = \tau_t(a_1) + \alpha \tau_t(a_2) = \tau_t(a_1 + \alpha a_2).
\end{align}
Moreover, the function $z \mapsto \eta(f_1(z) + \alpha f_2(z))$ is analytic for every $\eta \in X*$. Thus $a_1 + \alpha a_2$ is entire analytic. Therefore the set of entire analytic elements in $X$, denoted $X_\tau$, is a subspace of $X$. For $a_1, a_2 \in X_\tau$, $\alpha, z \in \mathbb{C}$, it follows from \eqref{eqn:entirevectorspace} that $\tau_z(a_1 + \alpha a_2) = \tau_z(a_1) + \tau_z(a_2)$.

Later we will prove that $X_\tau$ is also dense in $X$, both in the $\sigma(X,X*)$-topology (see Proposition \ref{prop:analyticdense}) and with respect to the norm (see Corollary \ref{corollary:entirenormdense}).
\end{remark}

When $\tau$ defines a dynamics on a C$^*$-algebra $A$, $A_\tau$ is not only a vector space, but a $\ast$-subalgebra. We will prove this result in Lemma \ref{lemma:atausubalgebra} on page \pageref{lemma:atausubalgebra}.

\begin{lemma}
\label{lemma:gaussian}
Let $n$ be a positive integer, and $\delta > 0$. Then
\begin{align}
\sqrt{\frac{n}{\pi}} \int_{-\infty}^{\infty} e^{-nt^2} dt &= 1, \label{eqn:gaussian1}\\
\sqrt{\frac{n}{\pi}} \int_{\vert t \vert \geq \delta} e^{-nt^2} dt &= \frac{1}{\sqrt{\pi}} \int_{\vert t \vert \geq \sqrt{n} \delta} e^{-t^2} dt \label{eqn:gaussian2}
.
\end{align}
Moreover, the second integral converges to zero as $n \rightarrow \infty$.
\end{lemma}
\begin{proof}
Let $\delta \geq 0$. Since the function $t \mapsto e^{-nt^2}$ is even, we have
\begin{align*}
\sqrt{\frac{n}{\pi}} \int_{\vert t \vert \geq \delta} e^{-nt^2} dt
&= 2 \sqrt{\frac{n}{\pi}} \int_{t \geq \delta} e^{-nt^2} dt\\
&= \frac{2}{\sqrt{\pi}} \int_{s \geq \sqrt{n} \delta} e^{-s^2} ds \text{, \hspace{5pt} by the change of variables $s = \sqrt{n}t$,}\\
&= \frac{1}{\sqrt{\pi}} \int_{\vert s \vert \geq \sqrt{n} \delta} e^{-s^2} ds
.
\end{align*}
Thus the equality $\eqref{eqn:gaussian2}$ follows. If $\delta = 0$, we have
\begin{align*}
\sqrt{\frac{n}{\pi}} \int_{-\infty}^{\infty} e^{-nt^2} dt
= \sqrt{\frac{n}{\pi}} \int_{\vert t \vert \geq 0} e^{-nt^2} dt
=  \frac{1}{\sqrt{\pi}} \int_{\vert s \vert \geq 0} e^{-s^2} ds
=  \frac{1}{\sqrt{\pi}} \int_{-\infty}^\infty e^{-s^2} ds
= 1
.
\end{align*}
Therefore the integral $\sqrt{\frac{n}{\pi}} \int_{\vert t \vert \geq \delta} e^{-nt^2} dt$ converges to zero as $n \rightarrow \infty$.
%%\begin{align*}
%%\frac{2}{\sqrt{\pi}} \int_{s \geq \sqrt{n} \delta} e^{-s^2} ds = \frac{1}{\sqrt{\pi}} \int_{\vert s \vert \geq \sqrt{n} \delta} e^{-s^2} ds
%%\end{align*}
\end{proof}

\begin{proposition} %P 1 pg 11 frausino
\label{prop:analyticdense}
If $\tau$ is a one-parameter $\sigma(X,X*)$-continuous group of isometries, and $a \in X$, define for $n = 1, 2, \hdots$,
\begin{align*}
a_n = \sqrt{\frac{n}{\pi}} \int_{-\infty}^{\infty} \tau_t(a)e^{-nt^2}dt
.
\end{align*}
Then, for each $n$, $a_n$ is an entire analytic element for $\tau$ and $\Vert a_n \Vert \leq \Vert a \Vert$. In addition,
\begin{align*}
\tau_z(a_n) = \sqrt{\frac{n}{\pi}} \int_{-\infty}^{\infty} \tau_t(a)e^{-n(t-z)^2}dt,
\end{align*}
for every $z \in \mathbb{C}$. Moreover, $a_n \rightarrow a$ on the $\sigma(X,X*)$ topology as $n \rightarrow \infty$. In particular, $X_\tau$, is a $\sigma(X,X*)$-dense subspace of $X$.
\end{proposition}
\begin{proof}
Let $a \in X$. Define for each $n = 1, 2, \hdots$ the function $f_n: \mathbb{C} \rightarrow X$ by
\begin{align*}
f_n(z) = \sqrt{\frac{n}{\pi}} \int_{-\infty}^{\infty} \tau_t(a) e^{-n(t-z)^2}dt
.
\end{align*}
This function is well-defined since $t \mapsto e^{-n(t-z)^2}$ is an integrable function, $\Vert \tau_t(a) \Vert \leq \Vert a \Vert$ for every $t$, and $t \mapsto e^{-n(t-z)^2} \tau_t(a)$ is continuous, then we apply Proposition \ref{prop:vectorintegralL1}. Note that for each $s \in \mathbb{R}$, we have
\begin{align*}
f_n(s)
&= \sqrt{\frac{n}{\pi}} \int_{-\infty}^{\infty} \tau_t(a) e^{-n(t-s)^2}dt\\
&= \sqrt{\frac{n}{\pi}} \int_{-\infty}^{\infty} \tau_{t+s}(a) e^{-nt^2}dt\\
&= \sqrt{\frac{n}{\pi}} \int_{-\infty}^{\infty} \tau_s \circ \tau_t(a) e^{-nt^2}dt\\
&= \tau_s \left(\sqrt{\frac{n}{\pi}} \int_{-\infty}^{\infty} \tau_t(a) e^{-nt^2}dt \right) \text{,\hspace{10pt} by Corollary \ref{corollary:operatorappliedtointegral},}\\
&= \tau_s(a_n).
\end{align*}

Let $\eta \in X*$. Let $z, z_0 \in \mathbb{C}$ such that $z \neq z_0$. By definition of $f_n$, it follows that
%We can use the inequality $\vert \eta(\tau_t(a)) \vert \leq \Vert \eta \Vert \Vert a \Vert$ and conclude that
\begin{align*}
\left\vert
    \frac{\eta(f_n(z)) - \eta(f_n(z_0))}{z - z_0}
    -\sqrt{\frac{n}{\pi}} \int_{-\infty}^\infty 2n(t-z)e^{-n(t-z)^2} \eta(\tau_t(a)) dt
\right\vert
\end{align*}
equals to
%\footnotesize
\begin{align*}
&\left\vert
     \sqrt{\frac{n}{\pi}} \int_{-\infty}^\infty \eta(\tau_t(a))  \left(\frac{e^{-n(t-z)^2} - e^{-n(t-z_0)^2}}{z-z_0}\right)dt
    -\sqrt{\frac{n}{\pi}} \int_{-\infty}^\infty 2n(t-z)e^{-n(t-z)^2} \eta(\tau_t(a)) dt
\right\vert\\
=& \sqrt{\frac{n}{\pi}} \left\vert \int_{-\infty}^\infty \left(\frac{e^{-n(t-z)^2} - e^{-n(t-z_0)^2}}{z-z_0} - 2n(t-z)e^{-n(t-z)^2}\right)\eta(\tau_t(a)) dt \right\vert\\
\leq& \sqrt{\frac{n}{\pi}} \int_{-\infty}^\infty \left\vert\frac{e^{-n(t-z)^2} - e^{-n(t-z_0)^2}}{z-z_0} - 2n(t-z)e^{-n(t-z)^2}\right\vert \vert \eta(\tau_t(a))\vert dt\\
\leq& \Vert \eta \Vert \Vert a \Vert \sqrt{\frac{n}{\pi}} \int_{-\infty}^\infty \left\vert\frac{e^{-n(t-z)^2} - e^{-n(t-z_0)^2}}{z-z_0} - 2n(t-z)e^{-n(t-z)^2}\right\vert dt
%\normalsize
,
\end{align*} since $\vert \eta(\tau_t(a)) \vert \leq \Vert \eta \Vert \Vert \tau_t(a) \Vert \leq \Vert \eta \Vert \Vert a \Vert$ for each $t$. This integral goes to zero when $z \rightarrow z_0$ and the entire analyticity follows. Also, $f_n(z) = \tau_z(a_n)$ for every $z \in \mathbb{C}$.

In addition, we have $\Vert a_n \Vert \leq \Vert a \Vert$. In fact,
\begin{align*}
\Vert a_n \Vert
&= \left\Vert \sqrt{\frac{n}{\pi}} \int_{-\infty}^{\infty} \tau_t(a)e^{-nt^2}dt \right\Vert\\
&\leq \sqrt{\frac{n}{\pi}} \int_{-\infty}^{\infty} \Vert \tau_t(a) \Vert e^{-nt^2}dt \text{,\hspace{10pt}from Lemma \ref{lemma:leqintnorm},}\\
&\leq \Vert a \Vert \sqrt{\frac{n}{\pi}} \int_{-\infty}^{\infty} e^{-nt^2}dt\\
&= \Vert a \Vert, \text{\hspace{10pt}from Lemma \ref{lemma:gaussian}.}
\end{align*}

Now we prove that $a_n$ converges to $a$ on the $\sigma(X,X*)$ topology. Let $\eta \in X*$. If $\eta = 0$ or $a = 0$, it follows that $\eta(a_n) = \eta(a) = 0$ for every $n$. Then we assume $\eta \neq 0$ and $a \neq 0$ without loss of generality.

Note that
\begin{align*}
\eta(a_n - a)
&= \eta(a_n) - \eta(a)\\
&= \sqrt{\frac{n}{\pi}} \int_{-\infty}^{\infty} \eta(\tau_t(a))e^{-nt^2}dt - \eta(a) \text{, \hspace{12pt}by definition of $a_n$,}\\
&= \sqrt{\frac{n}{\pi}} \int_{-\infty}^{\infty} (\eta(\tau_t(a)) - \eta(a))e^{-nt^2}dt,
%   \text{, \hspace{12pt}since $\sqrt{\frac{n}{\pi}} \int_{-\infty}^{\infty} e^{-nt^2}dt = 1$.}
\end{align*}
since $\sqrt{\frac{n}{\pi}} \int_{-\infty}^{\infty} e^{-nt^2}dt = 1$ by Lemma \ref{lemma:gaussian}.

Let $\varepsilon > 0$. Since the map $t \mapsto \tau_t(a)$ is continuous and $\eta \in X*$, there exists $\delta > 0$ such that
\begin{align}
\label{eqn:analyticdelta}
\text{$\vert t \vert < \delta$ implies $\vert \eta(\tau_t(a)) - \eta(a) \vert < \varepsilon/2$.}
\end{align}

Moreover, from Lemma \ref{lemma:gaussian}, there exists $N > 0$ such that, for every $n \geq N$, we have
\begin{align}
\label{eqn:analyticdelta2}
\sqrt{\frac{n}{\pi}} \int_{\vert t \vert \geq \delta} e^{-nt^2} dt
< \frac{\varepsilon}{4 \Vert \eta \Vert \Vert a \Vert}.
\end{align}

Then, for each $n \geq N$,
\begin{align*}
\vert \eta(a_n - a) \vert
=& \left\vert \sqrt{\frac{n}{\pi}} \int_{-\infty}^\infty e^{-nt^2} (\eta(\tau_t(a)) - \eta(a))dt \right\vert\\
\leq& \left\vert \sqrt{\frac{n}{\pi}} \int_{\vert t \vert \geq \delta} e^{-nt^2} (\eta(\tau_t(a)) - \eta(a))dt \right\vert
+ \left\vert \sqrt{\frac{n}{\pi}} \int_{\vert t \vert < \delta} e^{-nt^2} (\eta(\tau_t(a)) - \eta(a))dt \right\vert\\
\leq& \sqrt{\frac{n}{\pi}} \int_{\vert t \vert \geq \delta} e^{-nt^2} \vert \eta(\tau_t(a)) - \eta(a)) \vert dt
+     \sqrt{\frac{n}{\pi}} \int_{\vert t \vert < \delta} e^{-nt^2} \vert \eta(\tau_t(a)) - \eta(a)) \vert dt\\
\leq& \sqrt{\frac{n}{\pi}} \int_{\vert t \vert \geq \delta} e^{-nt^2} \vert \eta(\tau_t(a)) - \eta(a)) \vert dt
+     \frac{\varepsilon}{2}\sqrt{\frac{n}{\pi}} \int_{\vert t \vert < \delta} e^{-nt^2} dt, \text{\hspace{10pt}from $\eqref{eqn:analyticdelta}$,}\\
\leq& \sqrt{\frac{n}{\pi}} \int_{\vert t \vert \geq \delta} e^{-nt^2} \Vert \eta \Vert (\Vert \tau_t(a)\Vert + \Vert a \Vert) dt
+     \frac{\varepsilon}{2}\sqrt{\frac{n}{\pi}} \int_{\vert t \vert < \delta} e^{-nt^2} dt\\
\leq& \sqrt{\frac{n}{\pi}} \int_{\vert t \vert \geq \delta} e^{-nt^2} \Vert \eta \Vert (\Vert a\Vert + \Vert a \Vert) dt
+     \frac{\varepsilon}{2}\sqrt{\frac{n}{\pi}} \int_{\vert t \vert < \delta} e^{-nt^2} dt, \text{\hspace{7pt} since $\Vert \tau_t \Vert = 1$,}\\
=& 2\Vert \eta \Vert \Vert a \Vert \sqrt{\frac{n}{\pi}} \int_{\vert t \vert \geq \delta} e^{-nt^2} dt
+     \frac{\varepsilon}{2}\sqrt{\frac{n}{\pi}} \int_{\vert t \vert < \delta} e^{-nt^2} dt\\
\leq& 2\Vert \eta \Vert \Vert a \Vert \frac{\varepsilon}{4 \Vert \eta \Vert \Vert a \Vert}
+     \frac{\varepsilon}{2}\sqrt{\frac{n}{\pi}} \int_{\vert t \vert < \delta} e^{-nt^2} dt,
\text{\hspace{10pt}from $\eqref{eqn:analyticdelta2}$,}\\
\leq& 2\Vert \eta \Vert \Vert a \Vert \frac{\varepsilon}{4 \Vert \eta \Vert \Vert a \Vert}
+     \frac{\varepsilon}{2}\sqrt{\frac{n}{\pi}} \int_{-\infty}^{\infty} e^{-nt^2} dt,\\
=& \frac{\varepsilon}{2} + \frac{\varepsilon}{2}, \text{\hspace{10pt}from Lemma \ref{lemma:gaussian},}\\
=& \varepsilon.
\end{align*}
Hence $a_n \rightarrow a$ in the topology $\sigma(X,X*)$.
\end{proof}

%Frausino pg 13
\begin{remark}
Let $\tau$ be a one-parameter $\sigma(X,X*)$-continuous group of isometries. Given $\lambda$, we say that $a$ is analytic on the strip $I_\lambda$ if the conditions in Definition \ref{def:analytic} hold for $a$ and $\lambda$.

We say that $a \in X$ is {strongly analytic} on the strip $I_\lambda$ if there exists $f: I_\lambda \rightarrow X$ such that condition (i) in Definition \ref{def:analytic} is satisfied and the limit
\begin{align*}
\lim_{h \rightarrow 0} \frac{f(z + h) - f(z)}{h}
\end{align*}
exists for every $z \in I_\lambda$. We now show that these two notions are equivalent.
\end{remark}

\begin{lemma} %O Lucas me ajudou
\label{lemma:tauzplusw}
Let $\tau$ be a one-parameter $\sigma(X,X*)$-continuous group of isometries, and $a \in X_\tau$. Given $w \in \mathbb{C}$, $\tau_w(a) \in X_\tau$. Moreover, for every $z \in \mathbb{C}$ we have
\begin{align*}
\tau_{z+w}(a) = \tau_z \circ \tau_w(a).
\end{align*}
\end{lemma}
\begin{proof}
Let $a \in X_\tau$. Then there exists a function $f: \mathbb{C} \rightarrow X$ such that $f(t) = \tau_t(a)$ for every $t \in \mathbb{R}$, and $\eta \circ f$ is entire analytic for $\eta \in X*$.

Fix $s \in \mathbb{R}$. Let $f_s: \mathbb{C} \rightarrow X$ be the function defined by $f_s(w) = f(s+w)$. Then $\eta \circ f_s$ is entire analytic for all $\eta \in X*$.

Define $g: \mathbb{C} \rightarrow X$ by $g(w) = \tau_s \circ \tau_w(a)$. Note that $\eta \circ g$ is entire analytic for every $\eta \in X*$. In fact, given $ w \in \mathbb{C}$,
\begin{align*}
\eta \circ g(w)
= \eta \circ \tau_s \circ \tau_w(a)
= (\eta \circ \tau_s) \circ f(z).
\end{align*}
Since $\eta \circ \tau_s \in X*$ and $a$ is entire analytic, it follows that $(\eta \circ \tau_s) \circ f$ is entire analytic. Thus $\eta \circ g$ is entire analytic. Moreover, for $t \in \mathbb{R}$, we have
\begin{align*}
\eta \circ g(t) = \eta \circ \tau_s \circ \tau_t(a) = \eta \circ \tau_{s+t}(a) = \eta \circ f(t+s) = \eta \circ f_s(t).
\end{align*}
Thus $\eta \circ g$ and $\eta \circ f_s$ are entire analytic functions which agree on the real line. Thus, by the uniqueness theorem for analytic functions \cite[Theorem 6.9]{newman2010complex} we have $\eta \circ g = \eta \circ f_s$. $\eta$ is arbitrary and $X*$ separates poins in $X$, thus $g = f_s$. Therefore, for every $w \in \mathbb{C}$,
\begin{align}
\label{eqn:taustauw}
\tau_s \circ \tau_w(a) = \tau_{s+w}(a).
\end{align}

Now we fix $w \in \mathbb{C}$ and assume $s$ is a real variable. Define $f_w: \mathbb{C} \rightarrow X$ by $f_w(z) = f(w+z)$. Since $a$ is entire analytic, the function $\eta \circ f_w$ is entire analytic for every $\eta \in X*$. By equation \eqref{eqn:taustauw}, we have for all $t \in \mathbb{R}$ the equality
\begin{align*}
f_w(t) = f(w+t) = \tau_{t+w}(a) = \tau_t \circ \tau_w(a).
\end{align*}
Therefore $\tau_w(a)$ is entire analytic and
\begin{align*}
\tau_z\circ \tau_w(a) = f_w(z) = f(w+z) = \tau_{z+w}(a).
\end{align*}
\end{proof}

Let $\tau$ define a dynamics on a C$^*$-algebra. We say that a subset $A_1$ is {$\tau$-invariant} if $\tau_t(a) \in A_1$ for every $t \in \mathbb{R}, a \in A_1$.

\begin{lemma}
\label{lemma:atausubalgebra}
Let $(A, \tau)$ be a C$^*$-dynamical system. Then $A_\tau$ is a $\ast$-subalgebra which is $\tau$-invariant.
\end{lemma}
\begin{proof}
$A_\tau$ is a vector space by Remark \ref{remark:analyticvectorspace}. Moreover, $A_\tau$ is $\tau$-invariant by Lemma \ref{lemma:tauzplusw}.

Given $a, b \in A_\tau$, let $f_1, f_2: \mathbb{C} \rightarrow A$ be the functions such that $\eta \circ f_1, \eta \circ f_2$ are analytic for all $\eta \in A*$, and such that $f_1(t) = \tau_t(a)$, $f_2(t) = \tau_t(b)$ for every $t \in \mathbb{R}$.

Let $f = f_1f_2$. Then $\eta \circ f$ is analytic for all $\eta \in A*$. Moreover, given $t \in \mathbb{R}$,
\begin{align*}
f(t) = f_1(t)f_2(t) = \tau_t(a)\tau_t(b) = \tau_t(ab).
\end{align*}
Therefore $ab$ is entire analytic.

Define $f_1*$ by $f_1*(z) = f_1(\overline{z})*$. Then, for $t \in \mathbb{R}$,
\begin{align*}
f_1*(t) = f_1(t)* = \tau_t(a)* = \tau_t(a*).
\end{align*}
Given $\eta \in A*$, let $\eta_1 \in A*$ be defined by $\eta_1(b) = \overline{\eta(b*)}$ for $b \in A$. Then,
\begin{align*}
\eta \circ f_1*(z) = \eta(f_1(\overline{z})*) = \overline{\eta_1 \circ f(\overline{z})}.
\end{align*}
Note that the function $z \mapsto \overline{\eta_1 \circ f_1(\overline{z})}$ is analytic. In fact,
\begin{align*}
\lim_{h \rightarrow 0} \frac{\overline{\eta_1 \circ f_1(\overline{z} + \overline{h})} - \overline{\eta_1 \circ f_1(\overline{z})}}{h}
&= \overline{\left( \lim_{h \rightarrow 0} \frac{\eta_1 \circ f_1(\overline{z} + \overline{h}) - \eta_1 \circ f_1(\overline{z})}{\overline{h}} \right)}.
\end{align*}
This limit exists since $\eta_1 \circ f_1$ is analytic. Then $\eta \circ f_1*$ is analytic, and therefore $a*$ is entire analytic.
\end{proof}

%Frausino P2 pg 13
\begin{proposition}
\label{prop:weaklystronglyanalytic}
Let $\tau$ be a one-parameter $\sigma(X,X*)$-continuous group of isometries. Given $\lambda > 0$, $a \in X$ is analytic on the strip $I_\lambda$ if, and only if, $a$ is strongly analytic on $I_\lambda$.
\end{proposition}
\begin{proof}
Let $\eta \in X*$. Let $z_0 \in I_\lambda$. There exists $r > 0$ such that $D(z_0, r/2) \subset \overline{D(z_0, r)} \subset I_\lambda$.

Let $h, k \in D(0, r/2)$. Then $z_0+h, z_0+k \in D(z_0,r/2)$. Using Cauchy's integral formula and assuming $C = \partial D(z_0, r)$, we have
\begin{align*}
\eta(f(z_0  )) &= \frac{1}{2\pi i} \oint_C \frac{\eta(f(z))}{z - z_0} dz,\\
\eta(f(z_0+h)) &= \frac{1}{2\pi i} \oint_C \frac{\eta(f(z))}{z - z_0 - h} dz,\\
\eta(f(z_0+k)) &= \frac{1}{2\pi i} \oint_C \frac{\eta(f(z))}{z - z_0 - k} dz.
\end{align*}
Then
\begin{align}
& \eta\left( \frac{f(z_0+h) - f(z_0)}{h} - \frac{f(z_0+k) - f(z_0)}{k}\right) \nonumber\\
=& \frac{1}{2\pi i} \oint_C \eta(f(z))
\left[
    \frac{1}{h} \left( \frac{1}{z - z_0 - h} - \frac{1}{z - z_0} \right)
   -\frac{1}{k} \left( \frac{1}{z - z_0 - k} - \frac{1}{z - z_0} \right)
\right]dz \label{eqn:diffetaanalytic}
\end{align}

Note that $\frac{1}{a-b} - \frac{1}{a} = \frac{b}{a(a-b)}$ for $a, b$ complex numbers such that $a \neq b$ and $a \neq 0$. Applying this, we have that $\eqref{eqn:diffetaanalytic}$ equals to
\begin{align*}
&\frac{1}{2\pi i} \oint_C \eta(f(z))
\left[
    \frac{1}{h} \frac{h}{(z - z_0)(z - z_0 - h)}
   -\frac{1}{k} \frac{k}{(z - z_0)(z - z_0 - k)}
\right]dz\\
=&\frac{1}{2\pi i} \oint_C \eta(f(z))
\left[
    \frac{1}{(z - z_0)(z - z_0 - h)}
   -\frac{1}{(z - z_0)(z - z_0 - k)}
\right]dz\\
=&\frac{1}{2\pi i} \oint_C \frac{\eta(f(z))}{z - z_0}
\left[
    \frac{1}{z - z_0 - h}
   -\frac{1}{z - z_0 - k}
\right]dz\\
=&\frac{1}{2\pi i} \oint_C \frac{\eta(f(z))}{z - z_0}\frac{h-k}{(z - z_0 - h)(z - z_0 - k)}dz
\end{align*}

Note that for every $z$ such that $\vert z - z_0 \vert = r$, we have
\begin{align*}
     \vert z - z_0 - h \vert
\geq \vert z - z_0 \vert - \vert h \vert
\geq  r - \frac{r}{2}
= \frac{r}{2}   
\end{align*}
Thus
\begin{align}
\label{eqn:leq2h}
\frac{1}{\vert z - z_0 - h \vert} \leq \frac{2}{h}.
\end{align}
Analogously, $\frac{1}{\vert z - z_0 - k \vert} \leq \frac{2}{k}$. Recall that $C$ denotes the set of points $z$ satisfying $\vert z - z_0 \vert = r$. Therefore,

\begin{align*}
\left\vert
    \eta\left(
    \frac{f(z_0+h)-f(z_0)}{h} - \frac{f(z_0+k)-f(z_0)}{k}
    \right)
\right\vert
&= \left\vert \frac{1}{2\pi i} \oint_C \frac{\eta(f(z))}{z - z_0}\frac{h-k}{(z - z_0 - h)(z - z_0 - k)}dz \right\vert \\
&\leq r \max_{z \in C} \frac{\vert \eta(f(z)) \vert}{\vert z - z_0 \vert} \frac{\vert h - k \vert}{\vert z - z_0 - h \vert \vert z - z_0 - k \vert}\\
&\leq r\frac{4}{r^2} \max_{z \in C} \frac{\vert \eta(f(z)) \vert}{\vert z - z_0 \vert} \vert h - k \vert, \text{\hspace{10pt} by $\eqref{eqn:leq2h}$,}\\
&= \frac{4}{r^2} \max_{z \in C} \vert \eta(f(z)) \vert \vert h - k \vert\\
&\leq \frac{4}{r^2} \Vert \eta \Vert \max_{z \in C} \Vert f(z) \Vert \vert h - k \vert.
\end{align*}
Using the fact that $\Vert x \Vert = \sup_{\Vert \eta \Vert = 1} \Vert \eta(x) \Vert$ in a Banach space, we obtain
\begin{align*}
\left\vert \frac{f(z_0+h)-f(z_0)}{h} - \frac{f(z_0+k)-f(z_0)}{k} \right\vert
\leq \frac{4}{r^2} \max_{z \in C} \vert f(z) \vert \vert h-k \vert
.
\end{align*}
Since $X$ is complete, it follows that the limit
\begin{align*}
\lim_{h \rightarrow 0} \frac{f(z_0+h)-f(z_0)}{h}
\end{align*}
exists. In other words, $a$ is strongly analytic on $I_\lambda$.

Conversely, suppose that $a$ is strongly analytic on the strip $I_\lambda$. Let $z \in I_\lambda$. By hypothesis, there exists $x \in X$ such that
\begin{align*}
x = \lim_{h \rightarrow 0} \frac{f(z+h)-f(z)}{h}.
\end{align*}
Let $\eta \in X*$. Then
\begin{align*}
\eta(x)
= \eta\left( \lim_{h \rightarrow 0} \frac{f(z+h)-f(z)}{h} \right)
=  \lim_{h \rightarrow 0} \frac{\eta(f(z+h)) - \eta(f(z))}{h}.
\end{align*}
Hence $\eta \circ f$ is analytic at $z$. Since $z$ and $\eta$ are arbitrary, it follows that $a$ is analytic on $I_\lambda$.
\end{proof}

%Frausino C1 pg 13
\begin{corollary}
\label{corollary:entirenormdense}
If $\tau = \{ \tau_t \}_{t \in \mathbb{R}}$ is a one-parameter $\sigma(X,X*)$-continuous group of isometries, then $\tau$ is strongly continuous and $X_\tau$ is norm-dense in $X$.
\end{corollary}
\begin{proof}
Note that by strongly continuous, we mean that the map $t \mapsto \tau_t(a)$ is continuous with respect to the norm in $X$ for every $a \in X$.

Suppose $X_\tau$ is not dense in $X$. Let $H$ be the norm closure of $X_\tau$. By hypothesis, $H$ is a proper subspace of $X$. Let $y \in X \setminus H$. By the Hahn-Banach for the sets $H$ and $\{ y \}$, there exists a $\varphi \in X*$ such that
\begin{align}
\label{eqn:revarphi}
Re(\varphi(y)) < Re(\varphi(y)),
\text{\hspace{10pt} $h \in H$.}
\end{align}
Since $H$ is a proper subspace of $X$ and $\varphi$ is linear, $Re(\varphi(H))$ must be either $\{ 0 \}$ or $\mathbb{R}$. By equation $\eqref{eqn:revarphi}$, $Re(\varphi(H)) = \{ 0 \}$.

Note that $Im(\varphi(H)) = 0$. In fact, let $h \in H$. Then there is $\lambda \in \mathbb{R}$ such that $\varphi(h) = \lambda i$. Since $H$ is a complex vector space and $\varphi$ is linear, $ih \in H$ and $\varphi(ih) = \lambda$. It follows that $\lambda = 0$. The choice of $h$ is arbitrary, thus $Im(\varphi(H)) = \{ 0 \}$. Hence $\varphi$ is zero on $H$ and $\varphi(y) \neq 0$.

From Proposition \ref{prop:analyticdense}, $X_\tau$ is dense in $X$ with respect to the $\sigma(X,X*)$-topology. Since $H$ contains $X_\tau$, $H$ is also dense in $X$ in this topology. Thus there exists a sequence $\{ y_n \}$ in $H$ converging to $y$ in the $\sigma(X,X*)$-topology. Since $\varphi \in X*$, we have $\varphi(y_n) \rightarrow \varphi(y)$. This leads to a contradiction because $\varphi(y) \neq 0$ and $\varphi(y_n) = 0$ for every $n$. Therefore $H = X$, that is, $X_\tau$ is norm dense in $X$.

Now we show that $\tau$ is strongly continuous. Given $a \in X_\tau$, $z \in \mathbb{C}$, it follows from Proposition \ref{prop:weaklystronglyanalytic} that the limit
\begin{align*}
\lim_{h \rightarrow 0} \left\Vert \frac{\tau_{z+h}(a) - \tau_z(a)}{h} \right\Vert
\end{align*}
exists. Thus $\Vert \frac{\tau_{z+h}(a) - \tau_z(a)}{h} \Vert$ converges to zero as $h \rightarrow 0$, i.e., the function $z \mapsto \tau_z(a)$ is continuous with respect to the norm.

Now choose $a \in X$ arbitrary, fix $t \in \mathbb{R}$ and let $\varepsilon > 0$. Since $X_\tau$ is norm dense in $X$, there exists $a_\varepsilon \in X_\tau$ such that $\Vert a - a_\varepsilon \Vert < \varepsilon/3$.

Since $a_\varepsilon \in X_\tau$, there exists $\delta > 0$ such that for every $h \in \mathbb{R}$ with $\vert h \vert < \delta$, we have $\Vert \tau_{t+h}(a_\varepsilon) - \tau_t(a_\varepsilon) \Vert < \varepsilon/3$. Then
\begin{align*}
\Vert \tau_{t+h}(a) - \tau_t(a) \Vert
&\leq \Vert \tau_{t+h}(a) - \tau_{t+h}(a_\varepsilon) \Vert
+ \Vert \tau_{t+h}(a_\varepsilon) -  \tau_{t}(a_\varepsilon) \Vert
+ \Vert \tau_{t}(a_\varepsilon) -  \tau_{t}(a) \Vert\\
&\leq \Vert \tau_{t+h} \Vert \Vert a - a_\varepsilon \Vert
+ \Vert \tau_{t+h}(a_\varepsilon) -  \tau_{t}(a_\varepsilon) \Vert
+ \Vert \tau_{t} \Vert \Vert a_\varepsilon -  a \Vert\\
&= \Vert a - a_\varepsilon \Vert
+ \Vert \tau_{t+h}(a_\varepsilon) -  \tau_{t}(a_\varepsilon) \Vert
+ \Vert a_\varepsilon -  a \Vert\\
&< \frac{\varepsilon}{3}
+ \Vert \tau_{t+h}(a_\varepsilon) -  \tau_{t}(a_\varepsilon) \Vert
+ \frac{\varepsilon}{3}\\
&= \frac{2}{3}\varepsilon + \Vert \tau_{t+h}(a_\varepsilon) -  \tau_{t}(a_\varepsilon) \Vert\\
&\leq \frac{2}{3}\varepsilon + \frac{\varepsilon}{3}\\
&= \varepsilon.
\end{align*}
Then the map $t \mapsto \tau_t(a)$ is continuous. Since $a$ is arbitrary, $\tau$ is strongly continuous.
\end{proof}

\begin{definition} %Frausino D14 pg 14 (22 do pdf)
Let $(A,\tau)$ be C$^*$-dynamical system, $\varphi$ a state on $A$ and $\beta \in \mathbb{R}$. We say $\varphi$ is a $\tau$-$\text{KMS}_\beta$-state if
\begin{align*}
\varphi(a\tau_{i\beta}(b)) = \varphi(ba)
\end{align*}
for all $a, b$ in a $\ast$-subalgebra $A_0$ composed of entire analytic elements such that $A_0$ is norm-dense and $\tau$-invariant.
\end{definition}

When $\tau$ is implicit, we just say that $\varphi$ is a $\text{KMS}_\beta$-state in order to assert that $\varphi$ is a $\tau$-$\text{KMS}_\beta$-state. Moreover, if $\beta$ is fixed, we just say $\varphi$ is a KMS state.

\begin{remark}
If $\varphi$ is a KMS-state and $\beta = 0$, we have
\begin{align*}
\varphi(ab) = \varphi(ba),
\end{align*}
for every $a, b \in A_0$. From the continuity of $\varphi$, this equality holds for every $a, b \in A$. In this case, we say the state $\varphi$ is {tracial}.
\end{remark}

\begin{definition} %Quem definiu isso?
Let $(A, \tau)$ be a C$^*$-dynamical system. We say that $a \in A$ is {$\tau$-invariant} if $\tau_t(a) = a$ for every $a \in A$.
\end{definition}

\begin{definition} %Bratteli2 pg 76, pg 90 do pdf
Let $A$ be a C$^*$-algebra with dynamics $\tau$. We say that a state $\varphi$ on $A$ is {$\tau$-invariant} if $\varphi(\tau_t(a)) = \varphi(a)$ for every $a \in A$ and $t \in \mathbb{R}$.
\end{definition}

In this section we defined KMS-states as described in \cite{bratteli1996operator}. However, Neshveyev's theorem assumes a diferent definition of KMS-states in \cite{neshveyev2011kms}. The definition used is the item (ii) of the next theorem. Now we show an equivalence in the definition of KMS states when $\beta \neq 0$.

%KMS states are defined differently in \cite{bratteli1996operator} and \cite{neshveyev2011kms}. The following proposition shows that these two definitions are equivalent.
\begin{proposition} % => Frausino P4 pg 16 (24 do pdf)
\label{prop:kmsequivalence}
Let $A$ be a C$^*$-algebra with dynamics given by $\tau$ and let $\beta \in \mathbb{R} \setminus \{ 0 \}$. Given a state $\varphi$ on $A$, the following are equivalent:
\begin{itemize}
\item $\varphi$ is a $\text{KMS}_\beta$-state;
\item $\varphi$ is $\tau$-invariant and
\begin{align}
\label{eqn:kmsequivalence}
\varphi(a\tau_{i\beta}(b)) = \varphi(ba)
\end{align}
for a dense set of analytic elements $a,b \in A$.
\item Equation $\eqref{eqn:kmsequivalence}$ holds for every $a, b \in A_\tau$.
\end{itemize}
\end{proposition}
\begin{proof}
Assume $\beta > 0$ without loss of generality.

$(i) \Rightarrow (ii)$ Let $\varphi$ be a $\text{KMS}_\beta$-state. By definition, there exists a subalgebra $A_0$ composed of entire analytic elements such that $A_0$ is norm-dense, $\tau$-invariant and such that $\eqref{eqn:kmsequivalence}$ holds for every $a, b \in A_0$. Thus, we only need to show that $\varphi$ is $\tau$-invariant.

%First suppose $\beta \neq 0$. We can assume $\beta > 0$ without loss of generality.
Let $a \in A_0$. Define $f: \mathbb{C} \rightarrow \mathbb{C}$ by $f(z) = \varphi(\tau_z(a))$. Since $a$ is entire analytic and $\varphi \in A*$, it follows that $f$ is entire analytic.

Let $\{ u_\lambda \}_{\lambda \in \Lambda}$ be an approximate unit for $A$. Fix $\lambda \in \Lambda$. Since $A_0$ is norm dense in $A$, for every $\varepsilon > 0$ there exists $u_\lambda^{(\varepsilon)} \in A_0$ satisfying $\Vert u_\lambda^{(\varepsilon)} - u_\lambda \Vert < \varepsilon$. Both $u_\lambda^{(\varepsilon)}, a \in A_0$ and $\varphi$ is a $\text{KMS}_\beta$-state, then
\begin{align*}
\varphi(u_\lambda^{(\varepsilon)}\tau_{i\beta}(a)) = \varphi(au_\lambda^{(\varepsilon)}).
\end{align*}
Using the continuity of $\varphi$, we have
\begin{align*}
\varphi(u_\lambda\tau_{i\beta}(a)) = \varphi(au_\lambda),
\end{align*}
for every $\lambda \in \Lambda$. Again, using the continuity of $\varphi$ and the fact that $\{ u_\lambda \}_{\lambda \in \Lambda}$ is an approximate unit, we have
\begin{align*}
\varphi(\tau_{i\beta}(a))
= \lim_\lambda \varphi(u_\lambda \tau_{i\beta}(a))
= \lim_\lambda \varphi(au_\lambda)
= \varphi(a).
\end{align*}

Define $g: \mathbb{C} \rightarrow \mathbb{C}$ by $g(z) = \varphi(\tau_{z+i\beta}(a)) - \varphi(\tau_z(a))$. Since $a$ is entire analytic and $\varphi \in A*$, it follows that $g$ is entire analytic. Note that $g$ is zero on the real line. In fact, given $t \in \mathbb{R}$, we have by Lemma \ref{lemma:tauzplusw}
\begin{align*}
g(t)
= \varphi(\tau_{t+i\beta}(a)) - \varphi(\tau_t(a))
= \varphi(\tau_{i\beta}(\tau_t(a))) - \varphi(\tau_t(a))
= 0.
\end{align*}
Hence $g(z) = 0$ for every $z \in \mathbb{C}$, that is,
\begin{align}
\label{eqn:varphiperiodic}
\varphi(\tau_{z+i\beta}(a)) = \varphi(\tau_z(a)).
\end{align}
Let $f: \mathbb{C} \rightarrow \mathbb{C}$ be the analytic function defined by $f(z) = \varphi(\tau_z(a))$. From \eqref{eqn:varphiperiodic} it follows that $f$ is periodic, that is, for every $z \in \mathbb{C}$ there exists $s \in \mathbb{R}$ and $0 < t \leq \beta$ such that $f(z) = f(s + it)$. Then, for every $z \in \mathbb{C}$, we have
\begin{align*}
\vert f(z) \vert
&\leq \sup_{w \in \mathbb{C}} \vert f(w) \vert\\
&\leq \sup_{\substack{s \in \mathbb{R} \\ 0 < t \leq \beta}} \vert f(s + it) \vert\\
& = \sup_{\substack{s \in \mathbb{R} \\ 0 < t \leq \beta}} \vert \varphi(\tau_{s + it}(a)) \vert\\
& \leq \sup_{\substack{s \in \mathbb{R} \\ 0 < t \leq \beta}} \Vert \tau_{s + it}(a) \Vert\\
& = \sup_{\substack{s \in \mathbb{R} \\ 0 < t \leq \beta}} \Vert \tau_s(\tau_{it}(a)) \Vert
\text{,\hspace{10pt}by Lemma \ref{lemma:tauzplusw}},\\
& \leq \sup_{0 < t \leq \beta} \Vert \tau_{it}(a)) \Vert
\text{,\hspace{10pt}by definition of $\tau_s$ for $s \in \mathbb{R}$,}\\
& < \infty,
\end{align*}
since $f$ is continuous. Then $f$ is entire analytic and bounded. Therefore $f$ is constant. Thus, for every $z \in \mathbb{C}$, we have
\begin{align*}
\varphi(a) = f(0) = f(z) = \varphi(\tau_z(a)).
\end{align*}
In particular, for every $a \in A_0$ and $t \in \mathbb{R}$, we have
\begin{align}
\label{eqn:varphitauinvariant}
\varphi(\tau_t(a)) = \varphi(a).
\end{align}
Since $A_0$ is dense in $A$, it follows that $\eqref{eqn:varphitauinvariant}$ holds for every $t \in \mathbb{R}, a \in A$. Therefore $\varphi$ is $\tau$-invariant.

%Now suppose $\beta = 0$. Given $b \in A_0$, let $\lambda > 0$ such that $b$ is analytic on the strip $I_\lambda$. Given $a \in A$, define the analytic function $f: I_\lambda \rightarrow \mathbb{C}$ by $f(z) = \varphi(a\tau_z(b))$. Then, for each $t \in \mathbb

$(ii) \Rightarrow (iii)$ Let $\varphi$ be a $\tau$-invariant state and suppose that there exists a dense set $A_1$ of analytic elements such that $\eqref{eqn:kmsequivalence}$ holds for every $a, b \in A_1$. Let
\begin{align*}
\mathcal{D}_\beta = \{ z \in \mathbb{C} : 0 \leq \text{Im}(z) \leq \beta \}.
\end{align*}

Let $a, b \in A_\tau$. Define $\eta \in A*$ by $\eta(x) = \varphi(ax)$. Then we can define the entire analytic function $f:\mathbb{C} \rightarrow \mathbb{C}$ by $f(z) = \varphi(a\tau_z(b))$ because $f(z) = \eta(\tau_z(a))$.

Since $A_1$ is dense in $A$, there are sequences $\{ a_n \}_{n \in \mathbb{N}}$, $\{ b_n \}_{n \in \mathbb{N}}$ in $A_1$ such that $a_n \rightarrow a$ and $b_n \rightarrow b$. Let $a' = \sup_n \Vert a_n \Vert$, $b' = \sup_n \Vert b_n \Vert$. Both $a', b'$ are finite.

For every $n$, there exists $\lambda_n > \beta$ such that $b_n$ is analytic on the strip $I_{\lambda_n}$. So we can define the analytic function $f_n$ by $\widetilde{f}_n(z) = \varphi(a_n\tau_z(b_n))$ for $z \in I_{\lambda_n}$. Let $f_n = \widetilde{f}_n\vert_{\mathcal{D}_\beta}$. We will show that $\{ f_n \}_{n \in \mathbb{N}}$ is a Cauchy sequence with respect to the supremum norm.

In fact, given $n, m$, define $\lambda_{n,m} = \min \{ \lambda_n, \lambda_m \}$. Then $\widetilde{f}_n\vert_{I_{\lambda_{n,m}}} - \widetilde{f}_m\vert_{I_{\lambda_{n,m}}}$ is analytic on $I_{\lambda_{n,m}}$. Then the supremum of $\vert f_n - f_m \vert$ is attained on the boundary of $\mathcal{D}_\beta$. Hence, for each $z \in \mathcal{D}_\beta$, we have
\begin{align*}
\vert f_n(z) - f_m(z) \vert
\leq \max \left\{ \sup_{t \in \mathbb{R}} \vert f_n(t) - f_m(t) \vert, \sup_{t \in \mathbb{R}} \vert f_n(t+i\beta) - f_m(t+i\beta) \vert \right\}.
\end{align*}
However, for every $t \in \mathbb{R}$,
\begin{align*}
\vert f_n(t) - f_m(t) \vert
&= \vert \varphi(a_n\tau_t(b_n)) - \varphi(a_m\tau_t(b_m)) \vert\\
&\leq \vert \varphi(a_n\tau_t(b_n)) - \varphi(a_n\tau_t(b_m)) \vert
+ \vert \varphi(a_n\tau_t(b_m)) - \varphi(a_m\tau_t(b_m)) \vert\\
&\leq \Vert a_n\tau_t(b_n) - a_n\tau_t(b_m) \Vert
+ \Vert a_n\tau_t(b_m) - a_m\tau_t(b_m) \Vert\\
&\leq \Vert a_n \Vert \Vert \tau_t(b_n - b_m) \Vert
+ \Vert a_n - a_m \Vert \Vert \tau_t(b_m) \Vert\\
&\leq \Vert a_n \Vert \Vert b_n - b_m \Vert
+ \Vert a_n - a_m \Vert \Vert b_m \Vert\\
&\leq a' \Vert b_n - b_m \Vert
+ \Vert a_n - a_m \Vert b'.
\end{align*}
On the other hand,
\begin{align*}
\vert f_n(t+i\beta) - f_m(t+i\beta) \vert
&= \vert \varphi(a_n \tau_{t+i\beta}(b_n)) - \varphi(a_m \tau_{t+i\beta}(b_m)) \vert \\
&= \vert \varphi(\tau_t(b_n)a_n) - \varphi(\tau_t(b_m)a_m) \vert\\
&= \vert \varphi(\tau_t(b_n)a_n) - \varphi(\tau_t(b_n)a_m) \vert
+\vert \varphi(\tau_t(b_n)a_m) - \varphi(\tau_t(b_m)a_m) \vert\\
&\leq \Vert \tau_t(b_n)a_n - \tau_t(b_n)a_m \Vert
+\Vert \tau_t(b_n)a_m - \tau_t(b_m)a_m \Vert\\
&\leq \Vert \tau_t(b_n) \Vert \Vert  a_n - a_m \Vert
+\Vert \tau_t(b_n) - \tau_t(b_m)\Vert \Vert a_m \Vert\\
&\leq \Vert b_n \Vert \Vert  a_n - a_m \Vert
+\Vert b_n - b_m\Vert \Vert a_m \Vert\\
&\leq b'\Vert  a_n - a_m \Vert
+\Vert b_n - b_m\Vert a'.
\end{align*}
Therefore $\Vert f_n - f_m \Vert \leq b'\Vert  a_n - a_m \Vert +\Vert b_n - b_m\Vert a'$. Hence $\{ f_n \}_{n \in \mathbb{N}}$ is a Cauchy sequence and then this sequence converges to a continuous function $\widetilde{f}: \mathcal{D}_\beta \rightarrow \mathbb{C}$ which is analytic on the interior of $\mathcal{D}_\beta$. Note that for every $t \in \mathbb{R}$,
\begin{align*}
f(t) = \varphi(a\tau_t(b)) = \lim_{n \rightarrow \infty} \varphi(a_n\tau_t(b_n)) =\widetilde{f}(t),
\end{align*}
by the continuity of $\varphi$ and $\tau_t$. Therefore $f\vert_{\mathcal{D}_\beta} = \widetilde{f}$ by the uniqueness theorem for analytic functions. Moreover,
\begin{align*}
\varphi(a\tau_{i\beta}(b))
&= f(i\beta)\\
&= \lim_{n \rightarrow \infty} f_n(i\beta)\\
&= \lim_{n \rightarrow \infty} \varphi(a_n\tau_{i\beta}(b_n))\\
&= \lim_{n \rightarrow \infty} \varphi(b_n a_n)\\
&= \varphi(ba),
\end{align*}
for every $a, b \in A_\tau$. Therefore $\varphi$ is a $\text{KMS}_\beta$-state.

$(iii) \Rightarrow (i)$ From Lemma \ref{lemma:atausubalgebra}, $A_\tau$ is a $\ast$-subalgebra and is $\tau$-invariant. By Corollary \ref{corollary:entirenormdense}, $A_\tau$ is dense in $A$. Hence $\varphi$ is a $\text{KMS}_\beta$-state.
\end{proof}

\begin{remark}
Let $\varphi$ be a $\tau$-invariant state on a C$^*$-algebra $A$. In order to prove that $\varphi$ is a $\text{KMS}_\beta$-state, it suffices to show that $\varphi(a\tau_{i\beta}(b)) = \varphi(ba)$ in an arbitrary dense $\ast$-subalgebra of $A$. In fact, if $\beta \neq 0$, this follows directly from Proposition \ref{prop:kmsequivalence}. If $\beta = 0$, this follows from the continuity of $\varphi$.
\end{remark}

\begin{definition}
Given a C$^*$-algebra $A$ and a state $\varphi$ on $A$, we define the {centralizer} of $\varphi$ as the set
\begin{align*}
\{ a \in A : \varphi(ab) = \varphi(ba) \text{\hspace{10pt} for every $b \in A$} \}.
\end{align*}
\end{definition}

\begin{lemma}
\label{lemma:invariantisincentralizer}
Let $(A, \tau)$ be a C$^*$-dynamical system, $\beta > 0$, and $\varphi$ a $\tau\text{-KMS}_\beta$-state. Then, for every $a \in A$ such that $a$ is $\tau$-invariant, it follows that $a$ is in the centralizer of $\varphi$.
\end{lemma}
\begin{proof}
Let $a \in A$ be $\tau$-invariant. Then $\tau_t(a) = a$  for every $t$. Then we can define the function $f: \mathbb{C} \rightarrow A$ by $f(z) = a$. Then we have $f(t) = \tau_t(a)$ for every $t \in \mathbb{R}$. The function $f$ is constant, then $f$ is strongly analytic on $\mathbb{C}$. Then, by Proposition \ref{prop:weaklystronglyanalytic}, $a$ is entire analytic.

Let $b \in A_\tau$. Then,
\begin{align*}
\varphi(ba)
= \varphi(b\tau_{i\beta} (a)) 
= \varphi(ab),
\end{align*}
because $\varphi$ is  a $\tau\text{-KMS}_\beta$-state.
\end{proof}



Now we show that the set of KMS states, for a fixed $\beta>0$ is convex. Moreover, in order to describe all KMS states on a C$^*$-algebra, it is sufficient to find only its extremal KMS states.

\begin{lemma}
\label{lemma:kmsconvex}
Let $A$ be a C$^*$-algebra with dynamics $\tau$. Let $\beta \in \mathbb{R}$. The set of $\text{KMS}_\beta$-states is convex.
\end{lemma}
\begin{proof}
Let $A$ be a C$^*$-algebra with dynamics $\tau$. Fix $\beta \in \mathbb{R}$. Given $\varphi_1, \varphi_2$ KMS states, $0 < t < 1$, define $\varphi = t\varphi_1 + (1 - t)\varphi_2$. Now we show that $\varphi$ is a KMS state.
\begin{itemize}
\item $\varphi$ is a state.

Note that $\varphi$ is positive. In fact, given a positive element $a \in A$,
\begin{align*}
\varphi(a) = t\varphi_1(a) + (1-t)\varphi_2(a) \geq 0,
\end{align*}
since both $\varphi_1(a), \varphi_2(a) \geq 0$. Moreover, we prove that $\varphi$ has norm $1$. Applying Lemma \ref{thm:stateapproximateunit}, we have for every approximate unit $\{ u_\lambda \}_{\lambda \in \Lambda}$ of $A$,
\begin{align*}
\Vert \varphi \Vert
&= \lim_\lambda \varphi(u_\lambda)\\
&= \lim_\lambda \left(t\varphi_1(u_\lambda) + (1-t)\varphi_2(u_\lambda)\right)\\
&= t \lim_\lambda (\varphi_1(u_\lambda)) + (1-t) \lim_\lambda(\varphi_2(u_\lambda))\\
&= t \Vert \varphi_1\Vert + (1-t) \Vert \varphi_2 \Vert\\
&= t + (1-t) \\
&=1.
\end{align*}

\item $\varphi$ is KMS

Given $a, b \in A_\tau$,
\begin{align*}
\varphi(a\tau_{i\beta}(b))
= t\varphi_1(a\tau_{i\beta}(b)) + (1-t)\varphi_2(a\tau_{i\beta}(b))
= t\varphi_1(ba) + (1-t)\varphi_2(ba)
=\varphi(ba).
\end{align*}
\end{itemize}
\end{proof}

In order to prove that the  extremal KMS-states are sufficient to describe all KMS-states, we are going to use a the Krein-Milman theorem. But, before using this theorem, we show that the set of $\text{KMS}_\beta$-states is compact with respect to a topology we define below, the weak* topology. Results used in this part can be found on \cite{murphy2014c} and \cite{rudin1991functional}.

%Murphy pg 268
Let $X$ be a normed vector space. The {weak*-topology} on $X*$ is generated by the family of seminorms $p_x: X* \rightarrow \mathbb{R}$ such that $\eta \mapsto p_x(\eta) = \vert \eta(x) \vert$.

%functional analysis rudin T 3.15 pg 66
\begin{theorem} (The Banach-Alaoglu theorem) If $V$ is a neighborhood of $0$ in a normed vector space $X$ and if
\begin{align*}
K = \{ \eta \in X*: \vert \eta (x) \vert \leq 1 \text{\hspace{10pt} for every }x \in V \},
\end{align*}
then $K$ is compact in the weak*-topology.
\end{theorem}
In this case, we can also say that $K$ is {weak*-compact}.

\begin{lemma}
\label{lemma:kmscompact}
Let $A$ be a C$^*$-algebra with dynamics $\tau$. Let $\beta \in \mathbb{R}$. The set of $\text{KMS}_\beta$-states is compact in the weak*-topology.
\end{lemma}
\begin{proof}
Let $\widetilde{A}$ be the unitization of $A$. Let
\begin{align*}
\widetilde{K}
&= \{ \eta \in \widetilde{A}*: \vert \eta(a) \vert \leq 1 \text{\hspace{10pt} for $a \in A$ with $\Vert a \Vert \leq 1$}\}\\
&= \{ \eta \in \widetilde{A}*: \Vert \eta \Vert \leq 1 \}.
\end{align*}
It follows from the Banach-Alaoglu theorem that $\widetilde{K}$ is weak*-compact.

Let $\{ \varphi_\lambda \}_{\lambda \in \Lambda}$ be a net of $\text{KMS}_\beta$-states on $A$. Define for each $\lambda$, $\widetilde{\varphi}_\lambda$ the extension of $\varphi_\lambda$ on $\widetilde{A}$. Since each $\widetilde{\varphi}_\lambda \in \widetilde{K}$ and $\widetilde{K}$ is compact, there exists a subnet $\{ \widetilde{\varphi}_{\lambda_j} \}_{j \in J}$ converging to some $\widetilde{\varphi} \in \widetilde{K}$ in the weak*-topology. Hence, for every $a \in A$,
\begin{align*}
\varphi(a) = \lim_{j \in J} \varphi_{\lambda_j}(a).
\end{align*}
Also, since each $\widetilde{\varphi}_{\lambda_j}$ is a state 
\begin{align*}
\widetilde{\varphi}(1) = \lim_{j \in J} \widetilde{\varphi}_{\lambda_j}(1) = 1.
\end{align*}
It follows from Theorem \ref{thm:stateapproximateunit} that $\widetilde{\varphi}$ is a state. Hence $\varphi$ is a state. We will prove that $\varphi$ is a $\text{KMS}_\beta$-state.
%\begin{itemize}
%\item $\varphi$ is positive.

%Let $a$ be a positive element in $A$. Since $\varphi_{\lambda_j}(a) \geq 0$ for every $j \in J$, we have $\varphi(a) \geq 0$.

%\item $\Vert \varphi \Vert = 1$.

%Since $\varphi$ is positive and $\widetilde{\varphi}$ is the extension of $\varphi$ on $A$, we have
%\begin{align*}
%\Vert \varphi \Vert
%= \widetilde{\varphi}(1)
%= \lim_{j \in J} \widetilde{\varphi}_{\lambda_j}(1)
%= 1.
%\end{align*}

%\item $\varphi$ is a $\text{KMS}_\beta$-state

Let $a, b \in A_\tau$. Then
\begin{align*}
\varphi(a \tau_{i\beta}(b))
= \lim_{j \in J} \varphi_j(a \tau_{i\beta}(b))
= \lim_{j \in J} \varphi_j(ba)
= \varphi(ba).
\end{align*}
%\end{itemize}
Therefore the set of $\text{KMS}_\beta$-states is weak*-compact.
\end{proof}

We will use the fact that the set of KMS states is compact and convex to prove that the extremal KMS states are sufficient to describe all KMS states. Before proving this, we define some concepts about convex sets and state then state the Krein-Milman theorem. Here all results are defined for subsets of $X*$. For more general results, see \cite{murphy2014c}. 

%\begin{definition}
%Let $\Gamma$ be a non-empty family of seminorms on a vector space $X$. $X$ equipped with the topology generated by the seminorms in $\Gamma$ is called a {locally convex space}. $X$ i
%\end{definition}

%\begin{definition}
%Let $X$ be a normed vector space. Given a subset $S$ of $X*$, we define its {convex hull} the smallest convex set containing $S$. We denote this set by $\text{co}(S)$. We denote the closure of $\text{co}(S)$ with respect to the weak*-topology by $\overline{\text{co}}(S)$.
%\end{definition}
\begin{definition}
Let $X$ be a normed vector space. Given a subset $S$ of $X*$, $\overline{\text{co}}(S)$ denotes the closure of $\text{co}(S)$ with respect to the weak*-topology.
\end{definition}

Now we state the Krein-Milman theorem for $X*$.
\begin{theorem} %Murphy A.14 pg 273
Let $X$ be a normed vector space. Let $C \subset X*$ be a non-empty convex weak*-compact subset. Then the set $E$ of extreme points of $C$ is non-empty and
\begin{align*}
C = \overline{\text{co}}(E).
\end{align*}
Moreover, if $S$ is a closed subset of $C$ with respect to the weak*-topology such that $\overline{\text{co}}(S) = C$, then $S$ contains $E$.
\end{theorem}

%\begin{definition}
%Let $\tau$ define a dynamics on a C$^*$-algebra $A$. Fix $\beta > 0$. We say that a KMS state is extremal if it is a extreme point of the set of $\text{KMS}_\beta$-states on $A$.
%\end{definition}
%
Now we apply the Krein-Milman theorem to show that the extremal KMS states are sufficient to describe all KMS states on $A$.

\begin{corollary}
Let $A$ be a C$^*$-algebra and $\tau$ its dynamics. Fix $\beta > 0$. Let $C$ denote the set of $\text{KMS}_\beta$-states on $A$ and assume $C \neq \emptyset$. Let $E$ be the set of extremal $\text{KMS}_\beta$-states. Then $C = \overline{\text{co}}(E)$ and $E \neq \emptyset$.
\end{corollary}
\begin{proof}
It follows from Lemmas \ref{lemma:kmsconvex} and \ref{lemma:kmscompact} that $C$ is convex and compact. By hypothesis, $C \neq \emptyset$. Then we can apply the Krein-Milman theorem and the result follows.
\end{proof}




























==> ape-compactification.tex <==
\chapter{Alexandrov's Compactification} \label{ape:Alexandrov}

This appendix is mostly based on the books \cite{Kelley1955,Engelking1989}.

\begin{definition}[Compactifications] Let $X$ be a topological space. A compactification of the $X$ is a pair $(Y,c)$, where $Y$ is a compact topological space and $c:X \to Y$ is a homeomorphism onto its image (that is, a topological embedding) such that $X$ is dense on $Y$.
\end{definition}

\begin{definition}[Alexandrov's Compactification]\label{def:Alexandrov} Let $X$ be a non-compact topological space. Define an element $\infty \notin X$ and consider the set $X^*:= X \sqcup \{\infty\}$. The Alexandrov's compactification of $X$ is the topological space $X^*$ endowed with the topology
\begin{equation*}
    \tau^* = \tau \cup \{V \subseteq X^*:\infty \in V \text{ and } X\setminus V \text{ is compact and closed of } X \},
\end{equation*}
where $\tau$ is the topology on $X$.
\end{definition}

\begin{remark} If $X$ is Hausdorff, then we may remove the word `closed' on the definition above since in this case every compact is also closed (see Topological Appendix). Also, we have that
\begin{equation*}
    \{V \subseteq X^*:\infty \in V \text{ and } X\setminus V \text{ is compact and closed of } X \} = \{(X\setminus K)\cup\{\infty\}: K \text{ is compact and closed of } X\}.
\end{equation*}
\end{remark}

The next two results proves that the Alexandrov's compactification is well defined.

\begin{proposition} The family $\tau^*$ in the definition \ref{def:Alexandrov} is in fact a topology.
\end{proposition}

\begin{proof} We have $\emptyset \in \tau^*$ since $\emptyset \in \tau$. Also, $X^* \in \tau^*$ because $\infty \in X^*$ and $X\setminus X^* = \emptyset$ is closed and compact of $X$. Since $\tau$ is closed under unions and finite intersections, it is sufficient to prove that
\begin{itemize}
    \item[$(a)$] the unions and finite intersections of the elements in the form $(X\setminus K)\cup\{\infty\}$, $K$ compact and closed of $\tau$ are closed among themselves;
    \item[$(b)$] the union and finite intersection between an open set $U \subseteq X \subseteq X^*$ with an element in the form $(X\setminus K)\cup\{\infty\}$, $K$ compact and closed of $X$ is one of the these two kinds.
\end{itemize}

\textbf{Proof of $(a)$:} Let $I$ a set and $\{(X\setminus K_i)\cup\{\infty\}\}_{i \in I}$ a family of sets such that $K_i$ closed compact subset of $X$ for each $i \in I$. Then, 
\begin{equation*}
    \bigcup_{i \in I}(X\setminus K_i)\cup\{\infty\} =  \{\infty\} \cup \bigcup_{i \in I}(X\cap K_i^c) = \{\infty\} \cup \left(X\cap \bigcup_{i \in I} K_i^c\right) =  \left(X\setminus \left(\bigcap_{i \in I} K_i\right)\right) \cup  \{\infty\} \in \tau^*,
\end{equation*}
because the intersection of closed compact sets is also compact. Suppose now that $I$ is finite, then
\begin{equation*}
    \bigcap_{i \in I}(X\setminus K_i)\cup\{\infty\} =  \{\infty\} \cup \bigcap_{i \in I}(X\cap K_i^c) = \{\infty\} \cup \left(X\cap \bigcap_{i \in I} K_i^c\right) =  \left(X\setminus \left(\bigcup_{i \in I} K_i\right)\right) \cup  \{\infty\} \in \tau^*,
\end{equation*}
because the finite union of closed compact sets is also compact.

\textbf{Proof of $(b)$:} Let $U$ be an open set of $X$, then $F=X\setminus U$ is closed in $X$. For any set in the form $(X\setminus K)\cup \{\infty\}$, $K$ compact subset of $X$, we have
\begin{equation*}
    U \cup ((X\setminus K)\cup\{\infty\}) = U \cup (X\cap K^c)\cup\{\infty\} = ((U \cup X)\cap (U \cup K^c))\cup\{\infty\} = (X\cap (F \cap K)^c)\cup\{\infty\} = (X \setminus (F \cap K))\cup\{\infty\} \in \tau^*,
\end{equation*}
since $F \cap K$ is a closed subset of the compact set $K$, and therefore it is a compact set. Also, we have that
\begin{equation*}
    U \cap ((X\setminus K)\cup\{\infty\}) = U \cap ((X\cap K^c)\cup\{\infty\}) = ((U \cap (X\cap K^c))\cup(U \cap \{\infty\}) = (U \cap K^c) = U \setminus K \in \tau \subseteq \tau^*,
\end{equation*}
since an open set minus a closed set is also open.
\end{proof}

\begin{remark} It is straightforward that $X$ is a topological subspace of $X^*$.
\end{remark}

\begin{proposition} If $X$ is a non-compact topological space, then $X^*$ as in the definition \ref{def:Alexandrov} together with the natural inclusion map $i: X \to X^*$ is a compactification of $X$.
\end{proposition}

\begin{proof} We divide the proof in three parts.
\begin{itemize}
    \item[$(a)$] \textbf{$X^*$ is a compact space.} Let $\mathcal{U}$ an open cover of $X^*$, then there exists $V \in \mathcal{U}$ such that $\infty \in V$, and the topology of $X^*$ implies that $X^*\setminus V = X\setminus V$ is a compact subset of $X$, which is covered by $\mathcal{U}\setminus\{V\}$. Hence, there exists a finite subcover $\mathcal{U}'$ of $X\setminus V$ in $\mathcal{U}\setminus\{V\}$ and therefore $\mathcal{U}'\cup\{V\}$ is a finite subcover of $X^*$ in $\mathcal{U}$. Therefore $X^*$ is compact.
    \item[$(b)$] \textbf{$X$ is dense on $X^*$.} $X$ is compact if and only if $X^*\setminus X = \{\infty\}$ is an open set of $X^*$, i.e., $X$ is a closed subset of $X^*$, which is true if and only if $\overline{X}\neq X^*$, that is, $X$ is not dense in $X^*$. We conclude that $X$ is dense on $X^*$ if and only if $X$ is not compact.
    \item[$(c)$] \textbf{The map $i$ is a topological embedding.} Any inclusion map is a bijection onto its image. Also, $i(U) = i^{-1}(U) = U$ for any open set of $X$, and therefore $i$ is a homeomorphism onto its image.
\end{itemize}
\end{proof}

\begin{proposition}\label{prop:compact_iff_closed_compactification} Let $X$ be a non-compact Hausdorff space and $X^*$ its compactification. For any $K \subseteq X$, $K$ is a compact in $X$ if and only if $K$ is closed in $X^*$.
\end{proposition}

\begin{proof} Let $K \subseteq X$, that is, $K \subseteq X^*$ such that $\infty \in K^c$. $K$ is closed in $X^*$ if and only if $K^c$ is open, that is, $K^c = (X\setminus C) \cup \{\infty\}$, where $C$ is a compact subset of $X$, which is closed since $X$ is Hausdorff. we have the equivalences
\begin{equation*}
    K^c = (X\setminus C) \cup \{\infty\} \iff K = ((X\setminus C) \cup \{\infty\})^c = C.
\end{equation*}
Therefore, $K$ is closed in $X^*$ if and only if it is compact in $X$.
\end{proof}

\begin{theorem}[Uniqueness]\label{teo:uniqueness_Alexandrov} For any Hausdorff non-compact topological space, any compactification of this space done by including one point is the Alexandrov's compactification up to homeomorphisms.
\end{theorem}

\begin{proof} Let $Z$ be a compact space with topology $\tau_Z$. Suppose that $p \in Z$ is in the closure of $Y= Z\setminus \{p\}$ let $\tau_Y$ the subspace topology in $Y$. Suppose that $p \in U \in \tau_Z$ and let\footnote{Observe that $V\neq \emptyset$, otherwise $\{p\}$ would be an open set of $Z$, implying that $Y$ is closed and therefore $p$ would not be in the closure of $Y$, a contradiction.} $V = U \cap Y \in \tau_Y$. Then $Y \setminus V$ is closed in $Y$. Moreover, $Y \setminus V = Z \setminus U$ is also closed in $Z$ and hence compact in $Z$. By the proposition \ref{prop:compact_iff_closed_compactification}, we have that $Y\setminus V$ is compact in $Y$. We conclude that for every open neighborhood $U$ of $p$ it follows that $U^c$ is (closed) compact in $Y$, that is, for every $U$ s.t. $p \in U$ we have that $U = (Y\setminus K) \cup \{\infty\}$, and therefore $\tau_Z \subseteq \tau_Y^*$.

Now, take $K \subseteq Y$ (closed) compact in $Y$ and let $V = (Y\setminus K) \in \tau_Y$. We have that $Z \setminus K = (Y\cup{p})\setminus K = V\cup \{p\}$. We claim that $Z \setminus K \in \tau_Z$. Indeed, suppose that $Z \setminus K \notin \tau_Z$, hence $K$ is not closed subset of $Z$ and, by the proposition \ref{prop:compact_iff_closed_compactification}, $K$ is not compact in $Y$, a contradition. Then $\tau_Z \supseteq \tau_Y^*$. 

%\textbf{Claim:} $V \neq \emptyset$.
%\textit{Proof of the claim:} if $V = \emptyset$, then $U=\{p\}$ is an open subset of $Z$, and hence $Y$ is closed, a contradition because in this case $p$ is not in the closure of $Y$.


\end{proof}

\begin{definition}[Local compactness] A topological space $X$ is said to be locally compact if for every $x \in X$, there exists a compact neighborhood of $x$, that is, there exists $K_x$ compact set and $U_x$ open set such that $x \in U_x \subseteq K_x$.
\end{definition}

\begin{remark} Local compactness, as well as compactness, is a topological invariant, that is, it is preserved unde homeomorphisms.
\end{remark}

\begin{remark} If $X$ is a Hausdorff topological space, then $X$ is locally compact if and only if for every $x \in X$, there exists an open set $U_x$ such that $x \in U_x$ and $\overline{U_x}$ is compact. Indeed, if this is true, then $\overline{U_x}$ a compact neighborhood of $x$. On converse, in Hausdorff spaces, every compact set is closed. Hence, for a given open neighborhood $K_x$ of $x$ with $U_x$ being an open subset of $K_x$ containting $x$ we have that $\overline{U_x} \subseteq K_x$ since $K_x$ is closed, and then $\overline{U_x}$ is a closed subset of a compact set, therefore $\overline{U_x}$ is compact.
\end{remark}

\begin{proposition} Let $X$ be a non-compact topological space. $X$ is Hausdorff locally compact if and only if $X^*$ is Hausdorff.
\end{proposition}

\begin{proof} Suppose that $X$ is Hausdorff locally compact. Take $x,y \in X^*$. If, $x,y \in X$ then we can separate them by disjoint open sets of $X$, and the result follows since the $X$ is a subspace of $X^*$. Then suppose w.l.o.g. that $y = \infty$. Since $X$ is locally compact, there exists $K_x$ compact and $U_x$ open subsets of $X$ such that $x \in U_x \subseteq K_x$. It is straighforward that $U_x$ and $X^*\setminus K_x = X\setminus K_x$ are disjoint open sets of $X^*$ which separate $x$ from $y$. For the converse, suppose now that $X^*$ is Hausdorff, then $X$ is also Hausdorff, since it is homeomorphic to a Hausdorff subspace of $X^*$. Since $X^*$ is compact we have that $X$ is locally compact since it is homeomorphic to an open subset of a locally compact space.
\end{proof}


Consider the case of $X_A$ and $\widetilde{X}_A$ for $\mathcal{O}_A$ non-unital. We recall that $\Sigma_A$ is densely included in $\widetilde{X}_A$. Also, $\widetilde{X}_A$ is homeomorphic to a compact subspace of $\{0,1\}^\mathbb{F}$, and hence is a metric space. Moreover, $X_A$ is a metric subspace of $\widetilde{X}_A$, and since $\Sigma_A \subseteq X_A$, we get that $X_A$ is dense on $\widetilde{X}_A$. It is straightforward to notice that the inclusion map $X_A \xhookrightarrow{} \widetilde{X}_A$ is a homeomorphism on its image. We already know that $X_A$ is non-compact and $\widetilde{X}_A$ is compact. The theorem \ref{teo:uniqueness_Alexandrov} grants that $\widetilde{X}_A$ is the Alexandrov's compactification of $X_A$.


